LM-Polygraph: Uncertainty Estimation for Language Models

Recent advancements in the capabilities of large language models (LLMs) have paved the way for a myriad of groundbreaking applications in various fields. However, a significant challenge arises as these models often "hallucinate", i.e., fabricate facts without providing users an apparent means to discern the veracity of their statements. Uncertainty estimation (UE) methods are one path to safer, more responsible, and more effective use of LLMs. However, to date, research on UE methods for LLMs has been focused primarily on theoretical rather than engineering contributions. In this work, we tackle this issue by introducing LM-Polygraph, a framework with implementations of a battery of state-of-the-art UE methods for LLMs in text generation tasks, with unified program interfaces in Python. Additionally, it introduces an extendable benchmark for consistent evaluation of UE techniques by researchers, and a demo web application that enriches the standard chat dialog with confidence scores, empowering end-users to discern unreliable responses. LM-Polygraph is compatible with the most recent LLMs, including BLOOMz, LLaMA-2, ChatGPT, and GPT-4, and is designed to support future releases of similarly-styled LMs.

==> code/dataset.tex <==
\begin{minted}{python}
from lm_polygraph.utils.dataset import Dataset

dataset = Dataset.load(
    "../workdir/data/triviaqa.csv",
    "question", "answer",
    batch_size=4,
)
\end{minted}

==> code/results.tex <==
\begin{minted}{python}
results = man()
\end{minted}

==> code/ue_manager.tex <==
\begin{minted}{python}
from lm_polygraph.utils.manager import UEManager

man = UEManager(
    dataset,
    model,
    ue_methods,
    metrics,
    ue_metrics,
    loggers
)
\end{minted}

==> code/ue_methods.tex <==
\begin{minted}{python}
from lm_polygraph.estimators import *
from lm_polygraph.utils.processor import Logger
from lm_polygraph.ue_metrics import RiskCoverageCurveAUC
from lm_polygraph.generation_metrics import RougeMetric, BartScoreSeqMetric

ue_methods = [MaxProbabilitySeq(), 
              SemanticEntropy()]
ue_metrics = [RiskCoverageCurveAUC()]
metrics = [RougeMetric('rougeL'),
           BartScoreSeqMetric('rh'),]
loggers = [Logger()] 
\end{minted}



==> tables/camera_ready/llama.tex <==
\begin{table*}[!ht] \resizebox{\textwidth}{!}{\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{UE Method}} & \multicolumn{2}{c|}{\textbf{AESLC}} & \multicolumn{2}{c|}{\textbf{XSUM}} & \multicolumn{2}{c|}{\textbf{CoQA}} & \multicolumn{2}{c|}{\textbf{bAbiQA}} & \multicolumn{2}{c|}{\textbf{WMT14 De-En}} & \multicolumn{2}{c}{\textbf{WMT14 Fr-En}} \\ \cline{2-13}
    & \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore}&  \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore} \\\midrule
\midrule
            Maximum Sequence Probability &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.22$\pm$0.02 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.22$\pm$0.10 & \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.12$\pm$0.03 &          \cellcolor[rgb]{0.9246114999999999,0.8859735,0.6798645} 0.16$\pm$0.03 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.44$\pm$0.01 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.45$\pm$0.01 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.43$\pm$0.03 &                     \cellcolor[rgb]{0.9936465,0.942359,0.606668} 0.93$\pm$0.00 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.44$\pm$0.01 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.64$\pm$0.01 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.45$\pm$0.01 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.60$\pm$0.02 \\
                              Perplexity &                             \cellcolor[rgb]{0.824111,0.8052765,0.7274005} 0.12$\pm$0.02 &                    \cellcolor[rgb]{0.6548005,0.6701995000000001,0.712395} 0.01$\pm$0.10 &                   \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.13$\pm$0.03 &                    \cellcolor[rgb]{0.720905,0.722701,0.7268295} -0.04$\pm$0.03 &                    \cellcolor[rgb]{0.9034295,0.8686925,0.693842} 0.32$\pm$0.01 &                      \cellcolor[rgb]{0.818206,0.800632,0.728909} 0.18$\pm$0.01 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.43$\pm$0.03 &                     \cellcolor[rgb]{0.9936465,0.942359,0.606668} 0.93$\pm$0.00 &                             \cellcolor[rgb]{0.9976245,0.949192,0.6037805} 0.43$\pm$0.01 &                    \cellcolor[rgb]{0.939689,0.8983435,0.6681205} 0.46$\pm$0.01 &                    \cellcolor[rgb]{0.9773625,0.929323,0.6296825} 0.40$\pm$0.01 &          \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.41$\pm$0.02 \\
                      Mean Token Entropy &          \cellcolor[rgb]{0.8419749999999999,0.8193965000000001,0.7221255} 0.13$\pm$0.01 &                    \cellcolor[rgb]{0.6548005,0.6701995000000001,0.712395} 0.01$\pm$0.10 &                   \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.13$\pm$0.04 &                    \cellcolor[rgb]{0.704113,0.7086785,0.721285} -0.06$\pm$0.03 &          \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.33$\pm$0.01 &                     \cellcolor[rgb]{0.8045525,0.789908,0.731819} 0.16$\pm$0.01 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.43$\pm$0.04 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.99$\pm$0.00 &                             \cellcolor[rgb]{0.9976245,0.949192,0.6037805} 0.43$\pm$0.01 &          \cellcolor[rgb]{0.9246114999999999,0.8859735,0.6798645} 0.42$\pm$0.01 &           \cellcolor[rgb]{0.9842345,0.9349095000000001,0.620655} 0.41$\pm$0.01 &          \cellcolor[rgb]{0.9203465,0.8824810000000001,0.6828730000000001} 0.37$\pm$0.02 \\
            Pointwise Mutual Information &                                  \cellcolor[rgb]{0.5,0.578966,0.6787605} -0.07$\pm$0.01 &                                  \cellcolor[rgb]{0.5,0.578966,0.6787605} -0.07$\pm$0.10 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.16$\pm$0.04 &  \cellcolor[rgb]{0.8064884999999999,0.7914304999999999,0.731475} 0.05$\pm$0.03 &                         \cellcolor[rgb]{0.5,0.588041,0.7037885} -0.18$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.33$\pm$0.02 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.35$\pm$0.03 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -1.93$\pm$0.04 &                                  \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.47$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.91$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.59$\pm$0.01 &                                  \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.93$\pm$0.04 \\
Conditional Pointwise Mutual Information &                             \cellcolor[rgb]{0.824111,0.8052765,0.7274005} 0.12$\pm$0.01 &                    \cellcolor[rgb]{0.6548005,0.6701995000000001,0.712395} 0.01$\pm$0.10 &                   \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.13$\pm$0.04 &                    \cellcolor[rgb]{0.720905,0.722701,0.7268295} -0.04$\pm$0.03 &                    \cellcolor[rgb]{0.9034295,0.8686925,0.693842} 0.32$\pm$0.01 &                      \cellcolor[rgb]{0.818206,0.800632,0.728909} 0.18$\pm$0.01 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.43$\pm$0.03 &                     \cellcolor[rgb]{0.9936465,0.942359,0.606668} 0.93$\pm$0.00 &                             \cellcolor[rgb]{0.9976245,0.949192,0.6037805} 0.43$\pm$0.01 &                    \cellcolor[rgb]{0.939689,0.8983435,0.6681205} 0.46$\pm$0.01 &                    \cellcolor[rgb]{0.9773625,0.929323,0.6296825} 0.40$\pm$0.01 &          \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.41$\pm$0.02 \\
                                 P(True) &                               \cellcolor[rgb]{0.685215,0.693445,0.716714} 0.03$\pm$0.01 &                             \cellcolor[rgb]{0.775806,0.7674245,0.7357195} 0.09$\pm$0.09 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.17$\pm$0.03 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.26$\pm$0.04 &                     \cellcolor[rgb]{0.611132,0.640351,0.711957} -0.08$\pm$0.01 &                   \cellcolor[rgb]{0.6473345,0.6647655,0.711858} -0.11$\pm$0.02 &                   \cellcolor[rgb]{0.6473345,0.6647655,0.711858} -0.13$\pm$0.03 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.98$\pm$0.00 &                    \cellcolor[rgb]{0.717584,0.7198815000000001,0.725567} -0.07$\pm$0.01 &                  \cellcolor[rgb]{0.7515925,0.7484255,0.7361525} -0.11$\pm$0.01 &                  \cellcolor[rgb]{0.7664145,0.7600675,0.7362005} -0.02$\pm$0.01 &                   \cellcolor[rgb]{0.7987345,0.7853589999999999,0.7329105} 0.01$\pm$0.02 \\
                        P(True) Sampling &                                  \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.08$\pm$0.01 &                                  \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.08$\pm$0.10 &          \cellcolor[rgb]{0.5927265,0.6294569999999999,0.713394} -0.11$\pm$0.03 &                          \cellcolor[rgb]{0.5,0.581529,0.685804} -0.24$\pm$0.03 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.22$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.596683,0.7207805} -0.26$\pm$0.02 &                     \cellcolor[rgb]{0.8045525,0.789908,0.731819} 0.14$\pm$0.03 &           \cellcolor[rgb]{0.9977515,0.9519329999999999,0.606185} 0.97$\pm$0.00 &                           \cellcolor[rgb]{0.6492105,0.6661235,0.7119865} -0.21$\pm$0.01 &                   \cellcolor[rgb]{0.6746705,0.685207,0.7148425} -0.38$\pm$0.01 &                   \cellcolor[rgb]{0.6938525,0.700347,0.7186525} -0.19$\pm$0.01 &                     \cellcolor[rgb]{0.7142310000000001,0.71707,0.724432} -0.27$\pm$0.03 \\
            Monte Carlo Sequence Entropy &                              \cellcolor[rgb]{0.986557,0.936775,0.6173385} 0.21$\pm$0.02 &            \cellcolor[rgb]{0.96609,0.9200794999999999,0.6429400000000001} 0.20$\pm$0.09 &                   \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.13$\pm$0.04 &          \cellcolor[rgb]{0.9246114999999999,0.8859735,0.6798645} 0.16$\pm$0.03 &           \cellcolor[rgb]{0.9974235,0.946477,0.6017224999999999} 0.43$\pm$0.01 &           \cellcolor[rgb]{0.9974235,0.946477,0.6017224999999999} 0.44$\pm$0.01 &           \cellcolor[rgb]{0.9974235,0.946477,0.6017224999999999} 0.42$\pm$0.03 &                    \cellcolor[rgb]{0.975089,0.9274665,0.6325425} 0.84$\pm$0.01 &                              \cellcolor[rgb]{0.986557,0.936775,0.6173385} 0.41$\pm$0.01 &                     \cellcolor[rgb]{0.986557,0.936775,0.6173385} 0.59$\pm$0.01 &                    \cellcolor[rgb]{0.9773625,0.929323,0.6296825} 0.40$\pm$0.01 &                             \cellcolor[rgb]{0.975089,0.9274665,0.6325425} 0.52$\pm$0.02 \\
 Monte Carlo Normalized Sequence Entropy &                              \cellcolor[rgb]{0.8580885,0.832192,0.716193} 0.14$\pm$0.02 &                      \cellcolor[rgb]{0.7142310000000001,0.71707,0.724432} 0.05$\pm$0.09 &                    \cellcolor[rgb]{0.9705735,0.923765,0.6379075} 0.14$\pm$0.03 &                   \cellcolor[rgb]{0.7479565,0.745538,0.7358755} -0.01$\pm$0.03 &  \cellcolor[rgb]{0.8867430000000001,0.8551865000000001,0.703211} 0.30$\pm$0.01 &                     \cellcolor[rgb]{0.8045525,0.789908,0.731819} 0.16$\pm$0.01 &                     \cellcolor[rgb]{0.9616395,0.916411,0.647622} 0.37$\pm$0.04 &            \cellcolor[rgb]{0.972827,0.9256139999999999,0.635266} 0.83$\pm$0.01 &                             \cellcolor[rgb]{0.9976245,0.949192,0.6037805} 0.43$\pm$0.01 &           \cellcolor[rgb]{0.9418599999999999,0.900129,0.6662995} 0.47$\pm$0.01 &                    \cellcolor[rgb]{0.9773625,0.929323,0.6296825} 0.40$\pm$0.01 &                    \cellcolor[rgb]{0.9418599999999999,0.900129,0.6662995} 0.43$\pm$0.02 \\
                        Semantic Entropy &                              \cellcolor[rgb]{0.986557,0.936775,0.6173385} 0.21$\pm$0.02 & \cellcolor[rgb]{0.9484090000000001,0.9055150000000001,0.6604909999999999} 0.19$\pm$0.09 &                   \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.13$\pm$0.04 & \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.17$\pm$0.03 &           \cellcolor[rgb]{0.9974235,0.946477,0.6017224999999999} 0.43$\pm$0.01 &           \cellcolor[rgb]{0.9974235,0.946477,0.6017224999999999} 0.44$\pm$0.01 &                     \cellcolor[rgb]{0.9912485,0.940504,0.610439} 0.41$\pm$0.04 &   \cellcolor[rgb]{0.96609,0.9200794999999999,0.6429400000000001} 0.79$\pm$0.01 &                             \cellcolor[rgb]{0.979642,0.9311825,0.6267815} 0.40$\pm$0.01 &                    \cellcolor[rgb]{0.979642,0.9311825,0.6267815} 0.57$\pm$0.01 &            \cellcolor[rgb]{0.972827,0.9256139999999999,0.635266} 0.39$\pm$0.01 &                             \cellcolor[rgb]{0.9705735,0.923765,0.6379075} 0.51$\pm$0.02 \\
              Lexical Similarity Rouge-1 &                            \cellcolor[rgb]{0.9289045,0.8894845,0.6766295} 0.18$\pm$0.02 &                     \cellcolor[rgb]{0.8764430000000001,0.846883,0.708236} 0.15$\pm$0.10 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.16$\pm$0.03 &                     \cellcolor[rgb]{0.8908975,0.858537,0.700983} 0.13$\pm$0.03 &          \cellcolor[rgb]{0.8784875,0.8485355,0.7073294999999999} 0.29$\pm$0.01 & \cellcolor[rgb]{0.9182144999999999,0.8807415000000001,0.6843735} 0.33$\pm$0.01 &                     \cellcolor[rgb]{0.812327,0.796017,0.7302915} 0.15$\pm$0.04 &          \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.51$\pm$0.02 &                     \cellcolor[rgb]{0.972827,0.9256139999999999,0.635266} 0.39$\pm$0.01 &                     \cellcolor[rgb]{0.9616395,0.916411,0.647622} 0.52$\pm$0.01 &   \cellcolor[rgb]{0.96609,0.9200794999999999,0.6429400000000001} 0.38$\pm$0.01 & \cellcolor[rgb]{0.9484090000000001,0.9055150000000001,0.6604909999999999} 0.45$\pm$0.02 \\
              Lexical Similarity Rouge-2 &                            \cellcolor[rgb]{0.9289045,0.8894845,0.6766295} 0.18$\pm$0.02 &                   \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.16$\pm$0.10 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.16$\pm$0.03 &                     \cellcolor[rgb]{0.8702945,0.84195,0.7110655} 0.11$\pm$0.03 &                     \cellcolor[rgb]{0.690415,0.697582,0.7178265} 0.03$\pm$0.01 &                   \cellcolor[rgb]{0.5825565,0.6239825,0.714454} -0.20$\pm$0.02 &                      \cellcolor[rgb]{0.75527,0.7513215,0.736275} 0.06$\pm$0.03 &         \cellcolor[rgb]{0.7968109999999999,0.7838485,0.7332005} -0.14$\pm$0.03 &                             \cellcolor[rgb]{0.979642,0.9311825,0.6267815} 0.40$\pm$0.01 &                   \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.50$\pm$0.01 &   \cellcolor[rgb]{0.96609,0.9200794999999999,0.6429400000000001} 0.38$\pm$0.01 &                            \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.46$\pm$0.02 \\
              Lexical Similarity Rouge-L &                   \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.16$\pm$0.02 &                   \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.16$\pm$0.10 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.16$\pm$0.04 &                     \cellcolor[rgb]{0.8908975,0.858537,0.700983} 0.13$\pm$0.03 &          \cellcolor[rgb]{0.8784875,0.8485355,0.7073294999999999} 0.29$\pm$0.01 & \cellcolor[rgb]{0.9182144999999999,0.8807415000000001,0.6843735} 0.33$\pm$0.01 &                     \cellcolor[rgb]{0.812327,0.796017,0.7302915} 0.15$\pm$0.04 &          \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.51$\pm$0.02 &            \cellcolor[rgb]{0.96833,0.9219204999999999,0.6404380000000001} 0.38$\pm$0.01 &                   \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.50$\pm$0.01 &                     \cellcolor[rgb]{0.9616395,0.916411,0.647622} 0.37$\pm$0.01 &                    \cellcolor[rgb]{0.9572035,0.9127609999999999,0.652174} 0.47$\pm$0.02 \\
                 Lexical Similarity BLEU &          \cellcolor[rgb]{0.8419749999999999,0.8193965000000001,0.7221255} 0.13$\pm$0.02 &                             \cellcolor[rgb]{0.775806,0.7674245,0.7357195} 0.09$\pm$0.10 &                      \cellcolor[rgb]{0.98889,0.9386405,0.613977} 0.15$\pm$0.04 &            \cellcolor[rgb]{0.8379905000000001,0.816234,0.723368} 0.08$\pm$0.03 &                     \cellcolor[rgb]{0.8560525,0.83058,0.7170585} 0.26$\pm$0.01 &                     \cellcolor[rgb]{0.864167,0.8370535,0.713777} 0.25$\pm$0.01 &            \cellcolor[rgb]{0.8764430000000001,0.846883,0.708236} 0.25$\pm$0.03 & \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.63$\pm$0.01 &                     \cellcolor[rgb]{0.972827,0.9256139999999999,0.635266} 0.39$\pm$0.01 &                   \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.50$\pm$0.01 &                     \cellcolor[rgb]{0.9616395,0.916411,0.647622} 0.37$\pm$0.01 &                    \cellcolor[rgb]{0.9572035,0.9127609999999999,0.652174} 0.47$\pm$0.02 \\
                              NumSemSets &                    \cellcolor[rgb]{0.7589600000000001,0.754227,0.7363535} 0.08$\pm$0.01 &                    \cellcolor[rgb]{0.7589600000000001,0.754227,0.7363535} 0.08$\pm$0.10 &                     \cellcolor[rgb]{0.7948765,0.782341,0.733545} 0.03$\pm$0.03 &  \cellcolor[rgb]{0.8601110000000001,0.833809,0.7154024999999999} 0.10$\pm$0.03 &            \cellcolor[rgb]{0.816253,0.7990900000000001,0.729334} 0.21$\pm$0.01 &                      \cellcolor[rgb]{0.830041,0.809952,0.725767} 0.20$\pm$0.02 &            \cellcolor[rgb]{0.8379905000000001,0.816234,0.723368} 0.19$\pm$0.04 &          \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.51$\pm$0.02 &                            \cellcolor[rgb]{0.7776965,0.7689035,0.7355735} 0.05$\pm$0.01 &                     \cellcolor[rgb]{0.8045525,0.789908,0.731819} 0.06$\pm$0.01 &                  \cellcolor[rgb]{0.7664145,0.7600675,0.7362005} -0.02$\pm$0.01 &                   \cellcolor[rgb]{0.7987345,0.7853589999999999,0.7329105} 0.01$\pm$0.03 \\
       EigValLaplacian NLI Score entail. & \cellcolor[rgb]{0.9484090000000001,0.9055150000000001,0.6604909999999999} 0.19$\pm$0.01 &                   \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.17$\pm$0.09 &                    \cellcolor[rgb]{0.9034295,0.8686925,0.693842} 0.10$\pm$0.03 &                     \cellcolor[rgb]{0.9936465,0.942359,0.606668} 0.22$\pm$0.03 &                     \cellcolor[rgb]{0.864167,0.8370535,0.713777} 0.27$\pm$0.01 &           \cellcolor[rgb]{0.8846765,0.8535174999999999,0.704258} 0.28$\pm$0.01 &          \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.04$\pm$0.03 &          \cellcolor[rgb]{0.9505975,0.9073195000000001,0.6585105} 0.71$\pm$0.01 &                    \cellcolor[rgb]{0.9310525000000001,0.891247,0.6750055} 0.32$\pm$0.01 &           \cellcolor[rgb]{0.9310525000000001,0.891247,0.6750055} 0.44$\pm$0.01 & \cellcolor[rgb]{0.9182144999999999,0.8807415000000001,0.6843735} 0.29$\pm$0.01 &          \cellcolor[rgb]{0.9203465,0.8824810000000001,0.6828730000000001} 0.37$\pm$0.02 \\
       EigValLaplacian NLI Score Contra. &                     \cellcolor[rgb]{0.8764430000000001,0.846883,0.708236} 0.15$\pm$0.02 &          \cellcolor[rgb]{0.8419749999999999,0.8193965000000001,0.7221255} 0.13$\pm$0.10 &                     \cellcolor[rgb]{0.8702945,0.84195,0.7110655} 0.08$\pm$0.03 &                    \cellcolor[rgb]{0.9705735,0.923765,0.6379075} 0.20$\pm$0.03 &                     \cellcolor[rgb]{0.8560525,0.83058,0.7170585} 0.26$\pm$0.01 &           \cellcolor[rgb]{0.8846765,0.8535174999999999,0.704258} 0.28$\pm$0.01 &          \cellcolor[rgb]{0.7682765,0.7615335,0.7361759999999999} 0.08$\pm$0.04 &           \cellcolor[rgb]{0.9418599999999999,0.900129,0.6662995} 0.67$\pm$0.01 &                    \cellcolor[rgb]{0.9310525000000001,0.891247,0.6750055} 0.32$\pm$0.01 &           \cellcolor[rgb]{0.9310525000000001,0.891247,0.6750055} 0.44$\pm$0.01 &                    \cellcolor[rgb]{0.9139795,0.8772765,0.687146} 0.28$\pm$0.01 &                   \cellcolor[rgb]{0.9246114999999999,0.8859735,0.6798645} 0.38$\pm$0.02 \\
           EigValLaplacian Jaccard Score &                     \cellcolor[rgb]{0.8764430000000001,0.846883,0.708236} 0.15$\pm$0.02 &                             \cellcolor[rgb]{0.824111,0.8052765,0.7274005} 0.12$\pm$0.10 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.16$\pm$0.04 &                     \cellcolor[rgb]{0.8908975,0.858537,0.700983} 0.13$\pm$0.03 &                     \cellcolor[rgb]{0.8560525,0.83058,0.7170585} 0.26$\pm$0.01 &           \cellcolor[rgb]{0.8439785,0.820983,0.7214430000000001} 0.22$\pm$0.01 &                     \cellcolor[rgb]{0.850004,0.8257645,0.719312} 0.21$\pm$0.03 &           \cellcolor[rgb]{0.9418599999999999,0.900129,0.6662995} 0.67$\pm$0.02 &                             \cellcolor[rgb]{0.979642,0.9311825,0.6267815} 0.40$\pm$0.01 &   \cellcolor[rgb]{0.96833,0.9219204999999999,0.6404380000000001} 0.54$\pm$0.01 &            \cellcolor[rgb]{0.972827,0.9256139999999999,0.635266} 0.39$\pm$0.01 &                             \cellcolor[rgb]{0.9705735,0.923765,0.6379075} 0.51$\pm$0.02 \\
                DegMat NLI Score entail. &                   \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.16$\pm$0.01 &                   \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.16$\pm$0.09 & \cellcolor[rgb]{0.9203465,0.8824810000000001,0.6828730000000001} 0.11$\pm$0.04 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.23$\pm$0.03 &                       \cellcolor[rgb]{0.749776,0.74698,0.736016} 0.12$\pm$0.01 &                      \cellcolor[rgb]{0.710874,0.7142655,0.72332} 0.00$\pm$0.01 &                      \cellcolor[rgb]{0.75527,0.7513215,0.736275} 0.06$\pm$0.03 &         \cellcolor[rgb]{0.7987345,0.7853589999999999,0.7329105} -0.13$\pm$0.03 &                    \cellcolor[rgb]{0.9418599999999999,0.900129,0.6662995} 0.34$\pm$0.01 &                   \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.50$\pm$0.01 &                    \cellcolor[rgb]{0.939689,0.8983435,0.6681205} 0.33$\pm$0.01 &                            \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.46$\pm$0.02 \\
                DegMat NLI Score Contra. &                    \cellcolor[rgb]{0.7443485,0.742659,0.7355039999999999} 0.07$\pm$0.01 &                              \cellcolor[rgb]{0.729183,0.729776,0.7302285} 0.06$\pm$0.10 &  \cellcolor[rgb]{0.8867430000000001,0.8551865000000001,0.703211} 0.09$\pm$0.03 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.23$\pm$0.03 &                  \cellcolor[rgb]{0.6492105,0.6661235,0.7119865} -0.03$\pm$0.01 &                    \cellcolor[rgb]{0.6217425,0.647137,0.711507} -0.15$\pm$0.01 &            \cellcolor[rgb]{0.792958,0.780837,0.7338089999999999} 0.12$\pm$0.04 &           \cellcolor[rgb]{0.792958,0.780837,0.7338089999999999} -0.17$\pm$0.03 &                   \cellcolor[rgb]{0.9375285,0.8965624999999999,0.6698425} 0.33$\pm$0.01 &           \cellcolor[rgb]{0.963862,0.9182429999999999,0.6453055} 0.53$\pm$0.01 &           \cellcolor[rgb]{0.9440405000000001,0.9019195,0.664385} 0.34$\pm$0.01 &            \cellcolor[rgb]{0.96833,0.9219204999999999,0.6404380000000001} 0.50$\pm$0.02 \\
                    DegMat Jaccard Score &                     \cellcolor[rgb]{0.8764430000000001,0.846883,0.708236} 0.15$\pm$0.01 &                    \cellcolor[rgb]{0.808426,0.7929565000000001,0.7311185} 0.11$\pm$0.10 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.16$\pm$0.03 &            \cellcolor[rgb]{0.880548,0.8501920000000001,0.706319} 0.12$\pm$0.03 &                     \cellcolor[rgb]{0.864167,0.8370535,0.713777} 0.27$\pm$0.01 &                     \cellcolor[rgb]{0.8580885,0.832192,0.716193} 0.24$\pm$0.01 &            \cellcolor[rgb]{0.8764430000000001,0.846883,0.708236} 0.25$\pm$0.04 & \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.63$\pm$0.02 &                              \cellcolor[rgb]{0.9936465,0.942359,0.606668} 0.42$\pm$0.01 &            \cellcolor[rgb]{0.972827,0.9256139999999999,0.635266} 0.55$\pm$0.01 &            \cellcolor[rgb]{0.972827,0.9256139999999999,0.635266} 0.39$\pm$0.01 &            \cellcolor[rgb]{0.96833,0.9219204999999999,0.6404380000000001} 0.50$\pm$0.02 \\
          Eccentricity NLI Score entail. &                              \cellcolor[rgb]{0.986557,0.936775,0.6173385} 0.21$\pm$0.01 &                            \cellcolor[rgb]{0.9289045,0.8894845,0.6766295} 0.18$\pm$0.10 &  \cellcolor[rgb]{0.8867430000000001,0.8551865000000001,0.703211} 0.09$\pm$0.03 &                     \cellcolor[rgb]{0.9936465,0.942359,0.606668} 0.22$\pm$0.03 &           \cellcolor[rgb]{0.9974235,0.946477,0.6017224999999999} 0.43$\pm$0.01 &           \cellcolor[rgb]{0.9842345,0.9349095000000001,0.620655} 0.42$\pm$0.01 &          \cellcolor[rgb]{0.7853034999999999,0.7748475,0.7347965} 0.11$\pm$0.04 &           \cellcolor[rgb]{0.9572035,0.9127609999999999,0.652174} 0.74$\pm$0.01 &          \cellcolor[rgb]{0.9182144999999999,0.8807415000000001,0.6843735} 0.30$\pm$0.01 &                    \cellcolor[rgb]{0.9224785,0.884225,0.6813705} 0.41$\pm$0.01 &  \cellcolor[rgb]{0.8867430000000001,0.8551865000000001,0.703211} 0.23$\pm$0.01 &                   \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.29$\pm$0.02 \\
          Eccentricity NLI Score Contra. &                     \cellcolor[rgb]{0.8764430000000001,0.846883,0.708236} 0.15$\pm$0.01 &                    \cellcolor[rgb]{0.808426,0.7929565000000001,0.7311185} 0.11$\pm$0.10 &                     \cellcolor[rgb]{0.8399895,0.817813,0.722712} 0.06$\pm$0.03 &                     \cellcolor[rgb]{0.8908975,0.858537,0.700983} 0.13$\pm$0.03 & \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.36$\pm$0.01 &          \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.32$\pm$0.01 &   \cellcolor[rgb]{0.96833,0.9219204999999999,0.6404380000000001} 0.38$\pm$0.04 &          \cellcolor[rgb]{0.8784875,0.8485355,0.7073294999999999} 0.32$\pm$0.03 &                             \cellcolor[rgb]{0.872332,0.8435905,0.7101965} 0.22$\pm$0.01 &          \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.33$\pm$0.01 &            \cellcolor[rgb]{0.868244,0.8403145000000001,0.712014} 0.19$\pm$0.01 &                             \cellcolor[rgb]{0.8888255,0.8568595,0.702056} 0.28$\pm$0.02 \\
              Eccentricity Jaccard Score &                            \cellcolor[rgb]{0.9289045,0.8894845,0.6766295} 0.18$\pm$0.02 &                     \cellcolor[rgb]{0.8764430000000001,0.846883,0.708236} 0.15$\pm$0.09 &                      \cellcolor[rgb]{0.98889,0.9386405,0.613977} 0.15$\pm$0.03 &                      \cellcolor[rgb]{0.818206,0.800632,0.728909} 0.06$\pm$0.03 &                      \cellcolor[rgb]{0.98889,0.9386405,0.613977} 0.42$\pm$0.01 &           \cellcolor[rgb]{0.9842345,0.9349095000000001,0.620655} 0.42$\pm$0.01 &            \cellcolor[rgb]{0.8379905000000001,0.816234,0.723368} 0.19$\pm$0.04 &           \cellcolor[rgb]{0.9418599999999999,0.900129,0.6662995} 0.66$\pm$0.01 &                             \cellcolor[rgb]{0.9976245,0.949192,0.6037805} 0.43$\pm$0.01 &                   \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.50$\pm$0.01 &           \cellcolor[rgb]{0.9842345,0.9349095000000001,0.620655} 0.41$\pm$0.01 &                            \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.46$\pm$0.02 \\
          Mahalanobis Distance - Decoder &                            \cellcolor[rgb]{0.6397055,0.6593385,0.7115155} 0.00$\pm$0.01 &                             \cellcolor[rgb]{0.6217425,0.647137,0.711507} -0.01$\pm$0.10 &                       \cellcolor[rgb]{0.749776,0.74698,0.736016} 0.00$\pm$0.03 & \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.17$\pm$0.03 &  \cellcolor[rgb]{0.6566434999999999,0.6715599999999999,0.71256} -0.02$\pm$0.01 &           \cellcolor[rgb]{0.7443485,0.742659,0.7355039999999999} 0.06$\pm$0.01 & \cellcolor[rgb]{0.9182144999999999,0.8807415000000001,0.6843735} 0.31$\pm$0.04 &         \cellcolor[rgb]{0.7701534999999999,0.7630025,0.7360815} -0.30$\pm$0.03 &                    \cellcolor[rgb]{0.717584,0.7198815000000001,0.725567} -0.07$\pm$0.01 &                    \cellcolor[rgb]{0.753433,0.7498715,0.736216} -0.10$\pm$0.01 &            \cellcolor[rgb]{0.7142310000000001,0.71707,0.724432} -0.14$\pm$0.01 &                            \cellcolor[rgb]{0.730808,0.7312025,0.7309845} -0.21$\pm$0.03 \\
 Relative Mahalanobis Distance - Decoder &                               \cellcolor[rgb]{0.685215,0.693445,0.716714} 0.03$\pm$0.01 &                      \cellcolor[rgb]{0.7142310000000001,0.71707,0.724432} 0.05$\pm$0.09 &                     \cellcolor[rgb]{0.611132,0.640351,0.711957} -0.10$\pm$0.03 &                          \cellcolor[rgb]{0.5,0.581529,0.685804} -0.24$\pm$0.03 &                     \cellcolor[rgb]{0.64162,0.660695,0.7116055} -0.04$\pm$0.01 &                     \cellcolor[rgb]{0.737406,0.736916,0.7338405} 0.05$\pm$0.01 &                    \cellcolor[rgb]{0.5517005,0.610203,0.717895} -0.25$\pm$0.03 &                     \cellcolor[rgb]{0.864167,0.8370535,0.713777} 0.24$\pm$0.02 &                      \cellcolor[rgb]{0.7571129999999999,0.752773,0.73632} 0.01$\pm$0.01 &            \cellcolor[rgb]{0.816253,0.7990900000000001,0.729334} 0.10$\pm$0.01 &                     \cellcolor[rgb]{0.8580885,0.832192,0.716193} 0.17$\pm$0.01 &                    \cellcolor[rgb]{0.895058,0.8619049999999999,0.6987115} 0.30$\pm$0.02 \\
                           RDE - Decoder &                            \cellcolor[rgb]{0.516055,0.6005995,0.7203925} -0.05$\pm$0.01 &                                  \cellcolor[rgb]{0.5,0.590805,0.7109295} -0.06$\pm$0.10 &           \cellcolor[rgb]{0.808426,0.7929565000000001,0.7311185} 0.04$\pm$0.03 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.23$\pm$0.03 &           \cellcolor[rgb]{0.6639375000000001,0.677008,0.713335} -0.01$\pm$0.01 &                      \cellcolor[rgb]{0.75527,0.7513215,0.736275} 0.08$\pm$0.01 &          \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.30$\pm$0.04 &          \cellcolor[rgb]{0.7720345,0.764474,0.7359735000000001} -0.29$\pm$0.03 &                             \cellcolor[rgb]{0.722574,0.724113,0.7274425} -0.06$\pm$0.01 &                  \cellcolor[rgb]{0.7608215,0.7556835,0.7363195} -0.08$\pm$0.01 &                   \cellcolor[rgb]{0.739093,0.7383495,0.7344225} -0.08$\pm$0.01 &                            \cellcolor[rgb]{0.7479565,0.745538,0.7358755} -0.15$\pm$0.03 \\
                        HUQ-MD - Decoder &                    \cellcolor[rgb]{0.7443485,0.742659,0.7355039999999999} 0.07$\pm$0.01 &                             \cellcolor[rgb]{0.6217425,0.647137,0.711507} -0.01$\pm$0.10 &                   \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.13$\pm$0.03 &                    \cellcolor[rgb]{0.720905,0.722701,0.7268295} -0.04$\pm$0.03 &  \cellcolor[rgb]{0.8867430000000001,0.8551865000000001,0.703211} 0.30$\pm$0.01 &                     \cellcolor[rgb]{0.812327,0.796017,0.7302915} 0.17$\pm$0.01 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.43$\pm$0.04 &                     \cellcolor[rgb]{0.9936465,0.942359,0.606668} 0.93$\pm$0.00 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.21$\pm$0.01 & \cellcolor[rgb]{0.8459855000000001,0.8225724999999999,0.7207455} 0.19$\pm$0.01 &            \cellcolor[rgb]{0.8379905000000001,0.816234,0.723368} 0.13$\pm$0.01 &                              \cellcolor[rgb]{0.814288,0.797552,0.7298205} 0.06$\pm$0.03 \\
                       HUQ-RMD - Decoder &                    \cellcolor[rgb]{0.808426,0.7929565000000001,0.7311185} 0.11$\pm$0.02 &           \cellcolor[rgb]{0.700709,0.7058949999999999,0.7203539999999999} 0.04$\pm$0.10 &                   \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.13$\pm$0.03 &                    \cellcolor[rgb]{0.720905,0.722701,0.7268295} -0.04$\pm$0.03 &  \cellcolor[rgb]{0.8867430000000001,0.8551865000000001,0.703211} 0.30$\pm$0.01 &                     \cellcolor[rgb]{0.812327,0.796017,0.7302915} 0.17$\pm$0.01 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.43$\pm$0.03 &                     \cellcolor[rgb]{0.9936465,0.942359,0.606668} 0.93$\pm$0.00 &                             \cellcolor[rgb]{0.8888255,0.8568595,0.702056} 0.25$\pm$0.01 &                   \cellcolor[rgb]{0.8826115,0.8518525,0.7052935} 0.30$\pm$0.01 &          \cellcolor[rgb]{0.9505975,0.9073195000000001,0.6585105} 0.35$\pm$0.01 &                   \cellcolor[rgb]{0.9375285,0.8965624999999999,0.6698425} 0.42$\pm$0.02 \\
\bottomrule
\end{tabular}
}\caption{\label{tab:llama_2_results} PRR$\uparrow$ for the Llama v2 model with Rouge-L and BertScore as text quality metrics. Lighter color indicates better results.}\end{table*}

==> tables/camera_ready/llama_red_green.tex <==
\begin{table*}[!ht] \resizebox{\textwidth}{!}{\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{UE Method}} & \multicolumn{2}{c|}{\textbf{AESLC}} & \multicolumn{2}{c|}{\textbf{XSUM}} & \multicolumn{2}{c|}{\textbf{CoQA}} & \multicolumn{2}{c|}{\textbf{bAbiQA}} & \multicolumn{2}{c|}{\textbf{WMT14 De-En}} & \multicolumn{2}{c}{\textbf{WMT14 Fr-En}} \\ \cline{2-13}
    & \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore}&  \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore} \\\midrule
\midrule
            Maximum Sequence Probability &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.22$\pm$0.02 &   \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.22$\pm$0.10 & \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.12$\pm$0.03 &               \cellcolor[rgb]{0.9030769803177436,1.0,0.5807939874241916} 0.16$\pm$0.03 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.44$\pm$0.01 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.45$\pm$0.01 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.43$\pm$0.03 &                 \cellcolor[rgb]{0.8332775235331324,1.0,0.650593444208803} 0.93$\pm$0.00 &  \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.44$\pm$0.01 &  \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.64$\pm$0.01 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.45$\pm$0.01 &  \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.60$\pm$0.02 \\
                              Perplexity &                               \cellcolor[rgb]{1.0,0.9506172839506175,0.5} 0.12$\pm$0.02 &                  \cellcolor[rgb]{1.0,0.707377504378658,0.5} 0.01$\pm$0.10 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.13$\pm$0.03 &                             \cellcolor[rgb]{1.0,0.8072536204024094,0.5} -0.04$\pm$0.03 &                \cellcolor[rgb]{0.9276332924061464,1.0,0.5562376753357889} 0.32$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9421589986757232,0.5} 0.18$\pm$0.01 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.43$\pm$0.03 &                 \cellcolor[rgb]{0.8332775235331324,1.0,0.650593444208803} 0.93$\pm$0.00 & \cellcolor[rgb]{0.8259106299066116,1.0,0.6579603378353239} 0.43$\pm$0.01 & \cellcolor[rgb]{0.8858875618558619,1.0,0.5979834058860736} 0.46$\pm$0.01 &                \cellcolor[rgb]{0.8504669419950143,1.0,0.6334040257469211} 0.40$\pm$0.01 & \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.41$\pm$0.02 \\
                      Mean Token Entropy &                 \cellcolor[rgb]{0.9917773561037317,0.972403776325345,0.5} 0.13$\pm$0.01 &                  \cellcolor[rgb]{1.0,0.707377504378658,0.5} 0.01$\pm$0.10 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.13$\pm$0.04 &                             \cellcolor[rgb]{1.0,0.7790593361527619,0.5} -0.06$\pm$0.03 &                \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.33$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9224229997009699,0.5} 0.16$\pm$0.01 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.43$\pm$0.04 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.99$\pm$0.00 & \cellcolor[rgb]{0.8259106299066116,1.0,0.6579603378353239} 0.43$\pm$0.01 & \cellcolor[rgb]{0.9030769803177436,1.0,0.5807939874241916} 0.42$\pm$0.01 &                 \cellcolor[rgb]{0.8431000483684934,1.0,0.640770919373442} 0.41$\pm$0.01 & \cellcolor[rgb]{0.9079882427354242,1.0,0.5758827250065112} 0.37$\pm$0.02 \\
            Pointwise Mutual Information &               \cellcolor[rgb]{0.9996015518506869,0.5374428638557821,0.5} -0.07$\pm$0.01 & \cellcolor[rgb]{0.9996015518506869,0.5374428638557821,0.5} -0.07$\pm$0.10 &  \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.16$\pm$0.04 &                              \cellcolor[rgb]{1.0,0.9252424281259346,0.5} 0.05$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.5571788628305354,0.5} -0.18$\pm$0.01 &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.33$\pm$0.02 &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.35$\pm$0.03 &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -1.93$\pm$0.04 & \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.47$\pm$0.01 & \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.91$\pm$0.01 &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.59$\pm$0.01 & \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.93$\pm$0.04 \\
Conditional Pointwise Mutual Information &                               \cellcolor[rgb]{1.0,0.9506172839506175,0.5} 0.12$\pm$0.01 &                  \cellcolor[rgb]{1.0,0.707377504378658,0.5} 0.01$\pm$0.10 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.13$\pm$0.04 &                             \cellcolor[rgb]{1.0,0.8072536204024094,0.5} -0.04$\pm$0.03 &                \cellcolor[rgb]{0.9276332924061464,1.0,0.5562376753357889} 0.32$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9421589986757232,0.5} 0.18$\pm$0.01 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.43$\pm$0.03 &                 \cellcolor[rgb]{0.8332775235331324,1.0,0.650593444208803} 0.93$\pm$0.00 & \cellcolor[rgb]{0.8259106299066116,1.0,0.6579603378353239} 0.43$\pm$0.01 & \cellcolor[rgb]{0.8858875618558619,1.0,0.5979834058860736} 0.46$\pm$0.01 &                \cellcolor[rgb]{0.8504669419950143,1.0,0.6334040257469211} 0.40$\pm$0.01 & \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.41$\pm$0.02 \\
                                 P(True) &                               \cellcolor[rgb]{1.0,0.7553077876030589,0.5} 0.03$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.8873937374514077,0.5} 0.09$\pm$0.09 & \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.17$\pm$0.03 &               \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.26$\pm$0.04 &                              \cellcolor[rgb]{1.0,0.6526122431543425,0.5} -0.08$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.6964415395787946,0.5} -0.11$\pm$0.02 &                              \cellcolor[rgb]{1.0,0.6964415395787946,0.5} -0.13$\pm$0.03 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.98$\pm$0.00 &                 \cellcolor[rgb]{1.0,0.80161476355248,0.5} -0.07$\pm$0.01 &               \cellcolor[rgb]{1.0,0.8507411679268658,0.5} -0.11$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.8732965953265841,0.5} -0.02$\pm$0.01 &                \cellcolor[rgb]{1.0,0.9139647144260756,0.5} 0.01$\pm$0.02 \\
                        %P(True) Sampling &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.08$\pm$0.01 &  \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.08$\pm$0.10 &               \cellcolor[rgb]{1.0,0.6300568157546245,0.5} -0.11$\pm$0.03 &              \cellcolor[rgb]{0.9999475726119325,0.5430817207057116,0.5} -0.24$\pm$0.03 &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.22$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.5696526976803795,0.5} -0.26$\pm$0.02 &                               \cellcolor[rgb]{1.0,0.9224229997009699,0.5} 0.14$\pm$0.03 &                \cellcolor[rgb]{0.8234549986977713,1.0,0.6604159690441642} 0.97$\pm$0.00 &               \cellcolor[rgb]{1.0,0.6989192191037636,0.5} -0.21$\pm$0.01 &               \cellcolor[rgb]{1.0,0.7383912170532703,0.5} -0.38$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.7621427656029736,0.5} -0.19$\pm$0.01 &               \cellcolor[rgb]{1.0,0.7959759067025505,0.5} -0.27$\pm$0.03 \\
            Monte Carlo Sequence Entropy &                \cellcolor[rgb]{0.8406444171596532,1.0,0.6432265505822823} 0.21$\pm$0.02 &  \cellcolor[rgb]{0.8627450980392156,1.0,0.6211258697027198} 0.20$\pm$0.09 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.13$\pm$0.04 &               \cellcolor[rgb]{0.9030769803177436,1.0,0.5807939874241916} 0.16$\pm$0.03 &                \cellcolor[rgb]{0.8283662611154519,1.0,0.6555047066264836} 0.43$\pm$0.01 &                \cellcolor[rgb]{0.8283662611154519,1.0,0.6555047066264836} 0.44$\pm$0.01 &                \cellcolor[rgb]{0.8283662611154519,1.0,0.6555047066264836} 0.42$\pm$0.03 &                \cellcolor[rgb]{0.8529225732038546,1.0,0.6309483945380809} 0.84$\pm$0.01 & \cellcolor[rgb]{0.8406444171596532,1.0,0.6432265505822823} 0.41$\pm$0.01 & \cellcolor[rgb]{0.8406444171596532,1.0,0.6432265505822823} 0.59$\pm$0.01 &                \cellcolor[rgb]{0.8504669419950143,1.0,0.6334040257469211} 0.40$\pm$0.01 & \cellcolor[rgb]{0.8529225732038546,1.0,0.6309483945380809} 0.52$\pm$0.02 \\
 Monte Carlo Normalized Sequence Entropy & \cellcolor[rgb]{0.9753320683111952,0.9912854030501093,0.5085388994307402} 0.14$\pm$0.02 &                 \cellcolor[rgb]{1.0,0.7959759067025505,0.5} 0.05$\pm$0.09 & \cellcolor[rgb]{0.8578338356215351,1.0,0.6260371321204004} 0.14$\pm$0.03 &                             \cellcolor[rgb]{1.0,0.8451023110769363,0.5} -0.01$\pm$0.03 &                \cellcolor[rgb]{0.9409532313874316,1.0,0.5429177363545039} 0.30$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9224229997009699,0.5} 0.16$\pm$0.01 &                \cellcolor[rgb]{0.8676563604568961,1.0,0.6162146072850393} 0.37$\pm$0.04 &                \cellcolor[rgb]{0.8553782044126947,1.0,0.6284927633292406} 0.83$\pm$0.01 & \cellcolor[rgb]{0.8259106299066116,1.0,0.6579603378353239} 0.43$\pm$0.01 & \cellcolor[rgb]{0.8834319306470215,1.0,0.6004390370949139} 0.47$\pm$0.01 &                \cellcolor[rgb]{0.8504669419950143,1.0,0.6334040257469211} 0.40$\pm$0.01 & \cellcolor[rgb]{0.8834319306470215,1.0,0.6004390370949139} 0.43$\pm$0.02 \\
                        Semantic Entropy &                \cellcolor[rgb]{0.8406444171596532,1.0,0.6432265505822823} 0.21$\pm$0.02 &  \cellcolor[rgb]{0.8760650370205008,1.0,0.6078059307214347} 0.19$\pm$0.09 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.13$\pm$0.04 &               \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.17$\pm$0.03 &                \cellcolor[rgb]{0.8283662611154519,1.0,0.6555047066264836} 0.43$\pm$0.01 &                \cellcolor[rgb]{0.8283662611154519,1.0,0.6555047066264836} 0.44$\pm$0.01 &                \cellcolor[rgb]{0.8357331547419726,1.0,0.6481378129999628} 0.41$\pm$0.04 &                \cellcolor[rgb]{0.8627450980392156,1.0,0.6211258697027198} 0.79$\pm$0.01 &  \cellcolor[rgb]{0.848011310786174,1.0,0.6358596569557614} 0.40$\pm$0.01 &  \cellcolor[rgb]{0.848011310786174,1.0,0.6358596569557614} 0.57$\pm$0.01 &                \cellcolor[rgb]{0.8553782044126947,1.0,0.6284927633292406} 0.39$\pm$0.01 & \cellcolor[rgb]{0.8578338356215351,1.0,0.6260371321204004} 0.51$\pm$0.02 \\
              Lexical Similarity Rouge-1 &                \cellcolor[rgb]{0.8981657179000632,1.0,0.5857052498418722} 0.18$\pm$0.02 &  \cellcolor[rgb]{0.9532313874316329,1.0,0.5306395803103024} 0.15$\pm$0.10 &  \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.16$\pm$0.03 &                \cellcolor[rgb]{0.936041968969751,1.0,0.5478289987721844} 0.13$\pm$0.03 &                \cellcolor[rgb]{0.9507757562227926,1.0,0.5330952115191427} 0.29$\pm$0.01 &                \cellcolor[rgb]{0.9104438739442646,1.0,0.5734270937976709} 0.33$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9337007134008288,0.5} 0.15$\pm$0.04 &                \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.51$\pm$0.02 & \cellcolor[rgb]{0.8553782044126947,1.0,0.6284927633292406} 0.39$\pm$0.01 & \cellcolor[rgb]{0.8676563604568961,1.0,0.6162146072850393} 0.52$\pm$0.01 &                \cellcolor[rgb]{0.8627450980392156,1.0,0.6211258697027198} 0.38$\pm$0.01 & \cellcolor[rgb]{0.8760650370205008,1.0,0.6078059307214347} 0.45$\pm$0.02 \\
              %Lexical Similarity Rouge-2 &                \cellcolor[rgb]{0.8981657179000632,1.0,0.5857052498418722} 0.18$\pm$0.02 &  \cellcolor[rgb]{0.9335863377609107,1.0,0.5502846299810247} 0.16$\pm$0.10 &  \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.16$\pm$0.03 &               \cellcolor[rgb]{0.9605982810581537,1.0,0.5232726866837817} 0.11$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.7618010167029778,0.5} 0.03$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.6238198983297023,0.5} -0.20$\pm$0.02 &                               \cellcolor[rgb]{1.0,0.8563800247767954,0.5} 0.06$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.9111452860011109,0.5} -0.14$\pm$0.03 &  \cellcolor[rgb]{0.848011310786174,1.0,0.6358596569557614} 0.40$\pm$0.01 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.50$\pm$0.01 &                \cellcolor[rgb]{0.8627450980392156,1.0,0.6211258697027198} 0.38$\pm$0.01 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.46$\pm$0.02 \\
              Lexical Similarity Rouge-L &                \cellcolor[rgb]{0.9335863377609107,1.0,0.5502846299810247} 0.16$\pm$0.02 &  \cellcolor[rgb]{0.9335863377609107,1.0,0.5502846299810247} 0.16$\pm$0.10 &  \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.16$\pm$0.04 &                \cellcolor[rgb]{0.936041968969751,1.0,0.5478289987721844} 0.13$\pm$0.03 &                \cellcolor[rgb]{0.9507757562227926,1.0,0.5330952115191427} 0.29$\pm$0.01 &                \cellcolor[rgb]{0.9104438739442646,1.0,0.5734270937976709} 0.33$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9337007134008288,0.5} 0.15$\pm$0.04 &                \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.51$\pm$0.02 & \cellcolor[rgb]{0.8602894668303753,1.0,0.6235815009115601} 0.38$\pm$0.01 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.50$\pm$0.01 &                \cellcolor[rgb]{0.8676563604568961,1.0,0.6162146072850393} 0.37$\pm$0.01 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.47$\pm$0.02 \\
                 Lexical Similarity BLEU &                 \cellcolor[rgb]{0.9917773561037317,0.972403776325345,0.5} 0.13$\pm$0.02 &                 \cellcolor[rgb]{1.0,0.8873937374514077,0.5} 0.09$\pm$0.10 & \cellcolor[rgb]{0.8381887859508129,1.0,0.6456821817911225} 0.15$\pm$0.04 &               \cellcolor[rgb]{0.9935632697101611,0.9703532829253707,0.5} 0.08$\pm$0.03 & \cellcolor[rgb]{0.9777876995200356,0.9884659746251443,0.5060832682218999} 0.26$\pm$0.01 & \cellcolor[rgb]{0.9679651746846745,0.9986330044000171,0.5159057930572609} 0.25$\pm$0.01 &                \cellcolor[rgb]{0.9532313874316329,1.0,0.5306395803103024} 0.25$\pm$0.03 &                \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.63$\pm$0.01 & \cellcolor[rgb]{0.8553782044126947,1.0,0.6284927633292406} 0.39$\pm$0.01 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.50$\pm$0.01 &                \cellcolor[rgb]{0.8676563604568961,1.0,0.6162146072850393} 0.37$\pm$0.01 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.47$\pm$0.02 \\
                              NumSemSets &                               \cellcolor[rgb]{1.0,0.8620188816267249,0.5} 0.08$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.8620188816267249,0.5} 0.08$\pm$0.10 &                 \cellcolor[rgb]{1.0,0.908325857576146,0.5} 0.03$\pm$0.03 & \cellcolor[rgb]{0.9728764371023548,0.994104831475074,0.5109945306395806} 0.10$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.9393395702507584,0.5} 0.21$\pm$0.01 &                \cellcolor[rgb]{0.9996874651188749,0.9590755692255117,0.5} 0.20$\pm$0.02 &                \cellcolor[rgb]{0.9935632697101611,0.9703532829253707,0.5} 0.19$\pm$0.04 &                \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.51$\pm$0.02 &                \cellcolor[rgb]{1.0,0.8902131658763724,0.5} 0.05$\pm$0.01 &                \cellcolor[rgb]{1.0,0.9224229997009699,0.5} 0.06$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.8732965953265841,0.5} -0.02$\pm$0.01 &                \cellcolor[rgb]{1.0,0.9139647144260756,0.5} 0.01$\pm$0.03 \\
       EigValLaplacian NLI Score entail. &                \cellcolor[rgb]{0.8760650370205008,1.0,0.6078059307214347} 0.19$\pm$0.01 &  \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.17$\pm$0.09 & \cellcolor[rgb]{0.9276332924061464,1.0,0.5562376753357889} 0.10$\pm$0.03 &                \cellcolor[rgb]{0.8332775235331324,1.0,0.650593444208803} 0.22$\pm$0.03 & \cellcolor[rgb]{0.9679651746846745,0.9986330044000171,0.5159057930572609} 0.27$\pm$0.01 &                \cellcolor[rgb]{0.9434088625962718,1.0,0.5404621051456636} 0.28$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8366440258020421,0.5} 0.04$\pm$0.03 &                \cellcolor[rgb]{0.8736094058116604,1.0,0.6102615619302751} 0.71$\pm$0.01 & \cellcolor[rgb]{0.8957100866912229,1.0,0.5881608810507125} 0.32$\pm$0.01 & \cellcolor[rgb]{0.8957100866912229,1.0,0.5881608810507125} 0.44$\pm$0.01 &                \cellcolor[rgb]{0.9104438739442646,1.0,0.5734270937976709} 0.29$\pm$0.01 & \cellcolor[rgb]{0.9079882427354242,1.0,0.5758827250065112} 0.37$\pm$0.02 \\
       EigValLaplacian NLI Score Contra. &                \cellcolor[rgb]{0.9532313874316329,1.0,0.5306395803103024} 0.15$\pm$0.02 &   \cellcolor[rgb]{0.9917773561037317,0.972403776325345,0.5} 0.13$\pm$0.10 & \cellcolor[rgb]{0.9605982810581537,1.0,0.5232726866837817} 0.08$\pm$0.03 &               \cellcolor[rgb]{0.8578338356215351,1.0,0.6260371321204004} 0.20$\pm$0.03 & \cellcolor[rgb]{0.9777876995200356,0.9884659746251443,0.5060832682218999} 0.26$\pm$0.01 &                \cellcolor[rgb]{0.9434088625962718,1.0,0.5404621051456636} 0.28$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8761160237515488,0.5} 0.08$\pm$0.04 &                \cellcolor[rgb]{0.8834319306470215,1.0,0.6004390370949139} 0.67$\pm$0.01 & \cellcolor[rgb]{0.8957100866912229,1.0,0.5881608810507125} 0.32$\pm$0.01 & \cellcolor[rgb]{0.8957100866912229,1.0,0.5881608810507125} 0.44$\pm$0.01 &                \cellcolor[rgb]{0.9153551363619451,1.0,0.5685158313799904} 0.28$\pm$0.01 & \cellcolor[rgb]{0.9030769803177436,1.0,0.5807939874241916} 0.38$\pm$0.02 \\
           EigValLaplacian Jaccard Score &                \cellcolor[rgb]{0.9532313874316329,1.0,0.5306395803103024} 0.15$\pm$0.02 &                 \cellcolor[rgb]{1.0,0.9506172839506175,0.5} 0.12$\pm$0.10 &  \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.16$\pm$0.04 &                \cellcolor[rgb]{0.936041968969751,1.0,0.5478289987721844} 0.13$\pm$0.03 & \cellcolor[rgb]{0.9777876995200356,0.9884659746251443,0.5060832682218999} 0.26$\pm$0.01 &                 \cellcolor[rgb]{0.9917773561037317,0.972403776325345,0.5} 0.22$\pm$0.01 & \cellcolor[rgb]{0.9851545931465564,0.9800076893502501,0.5002232392008037} 0.21$\pm$0.03 &                \cellcolor[rgb]{0.8834319306470215,1.0,0.6004390370949139} 0.67$\pm$0.02 &  \cellcolor[rgb]{0.848011310786174,1.0,0.6358596569557614} 0.40$\pm$0.01 & \cellcolor[rgb]{0.8602894668303753,1.0,0.6235815009115601} 0.54$\pm$0.01 &                \cellcolor[rgb]{0.8553782044126947,1.0,0.6284927633292406} 0.39$\pm$0.01 & \cellcolor[rgb]{0.8578338356215351,1.0,0.6260371321204004} 0.51$\pm$0.02 \\
                DegMat NLI Score entail. &                \cellcolor[rgb]{0.9335863377609107,1.0,0.5502846299810247} 0.16$\pm$0.01 &  \cellcolor[rgb]{0.9335863377609107,1.0,0.5502846299810247} 0.16$\pm$0.09 & \cellcolor[rgb]{0.9079882427354242,1.0,0.5758827250065112} 0.11$\pm$0.04 &                \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.23$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.8479217395019011,0.5} 0.12$\pm$0.01 &                                \cellcolor[rgb]{1.0,0.790337049852621,0.5} 0.00$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8563800247767954,0.5} 0.06$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.9139647144260756,0.5} -0.13$\pm$0.03 & \cellcolor[rgb]{0.8834319306470215,1.0,0.6004390370949139} 0.34$\pm$0.01 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.50$\pm$0.01 &                \cellcolor[rgb]{0.8858875618558619,1.0,0.5979834058860736} 0.33$\pm$0.01 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.46$\pm$0.02 \\
                DegMat NLI Score Contra. &                               \cellcolor[rgb]{1.0,0.8394634542270069,0.5} 0.07$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.8213507625272333,0.5} 0.06$\pm$0.10 & \cellcolor[rgb]{0.9409532313874316,1.0,0.5429177363545039} 0.09$\pm$0.03 &                \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.23$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.6989192191037636,0.5} -0.03$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.6667093852791663,0.5} -0.15$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9055064291511813,0.5} 0.12$\pm$0.04 &                              \cellcolor[rgb]{1.0,0.9055064291511813,0.5} -0.17$\pm$0.03 & \cellcolor[rgb]{0.8883431930647021,1.0,0.5955277746772334} 0.33$\pm$0.01 & \cellcolor[rgb]{0.8652007292480559,1.0,0.6186702384938796} 0.53$\pm$0.01 &                \cellcolor[rgb]{0.8809762994381813,1.0,0.6028946683037542} 0.34$\pm$0.01 & \cellcolor[rgb]{0.8602894668303753,1.0,0.6235815009115601} 0.50$\pm$0.02 \\
                    DegMat Jaccard Score &                \cellcolor[rgb]{0.9532313874316329,1.0,0.5306395803103024} 0.15$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.9280618565508993,0.5} 0.11$\pm$0.10 &  \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.16$\pm$0.03 &                \cellcolor[rgb]{0.9483201250139524,1.0,0.535550842727983} 0.12$\pm$0.03 & \cellcolor[rgb]{0.9679651746846745,0.9986330044000171,0.5159057930572609} 0.27$\pm$0.01 & \cellcolor[rgb]{0.9753320683111952,0.9912854030501093,0.5085388994307402} 0.24$\pm$0.01 &                \cellcolor[rgb]{0.9532313874316329,1.0,0.5306395803103024} 0.25$\pm$0.04 &                \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.63$\pm$0.02 &  \cellcolor[rgb]{0.8332775235331324,1.0,0.650593444208803} 0.42$\pm$0.01 & \cellcolor[rgb]{0.8553782044126947,1.0,0.6284927633292406} 0.55$\pm$0.01 &                \cellcolor[rgb]{0.8553782044126947,1.0,0.6284927633292406} 0.39$\pm$0.01 & \cellcolor[rgb]{0.8602894668303753,1.0,0.6235815009115601} 0.50$\pm$0.02 \\
          Eccentricity NLI Score entail. &                \cellcolor[rgb]{0.8406444171596532,1.0,0.6432265505822823} 0.21$\pm$0.01 &  \cellcolor[rgb]{0.8981657179000632,1.0,0.5857052498418722} 0.18$\pm$0.10 & \cellcolor[rgb]{0.9409532313874316,1.0,0.5429177363545039} 0.09$\pm$0.03 &                \cellcolor[rgb]{0.8332775235331324,1.0,0.650593444208803} 0.22$\pm$0.03 &                \cellcolor[rgb]{0.8283662611154519,1.0,0.6555047066264836} 0.43$\pm$0.01 &                 \cellcolor[rgb]{0.8431000483684934,1.0,0.640770919373442} 0.42$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8997821350762528,0.5} 0.11$\pm$0.04 &                \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.74$\pm$0.01 & \cellcolor[rgb]{0.9104438739442646,1.0,0.5734270937976709} 0.30$\pm$0.01 &  \cellcolor[rgb]{0.905532611526584,1.0,0.5783383562153515} 0.41$\pm$0.01 &                \cellcolor[rgb]{0.9409532313874316,1.0,0.5429177363545039} 0.23$\pm$0.01 & \cellcolor[rgb]{0.9335863377609107,1.0,0.5502846299810247} 0.29$\pm$0.02 \\
          Eccentricity NLI Score Contra. &                \cellcolor[rgb]{0.9532313874316329,1.0,0.5306395803103024} 0.15$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.9280618565508993,0.5} 0.11$\pm$0.10 &  \cellcolor[rgb]{0.9917773561037317,0.972403776325345,0.5} 0.06$\pm$0.03 &                \cellcolor[rgb]{0.936041968969751,1.0,0.5478289987721844} 0.13$\pm$0.03 &                \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.36$\pm$0.01 &                \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.32$\pm$0.01 &                \cellcolor[rgb]{0.8602894668303753,1.0,0.6235815009115601} 0.38$\pm$0.04 &                \cellcolor[rgb]{0.9507757562227926,1.0,0.5330952115191427} 0.32$\pm$0.03 &  \cellcolor[rgb]{0.9581426498493135,1.0,0.525728317892622} 0.22$\pm$0.01 & \cellcolor[rgb]{0.9335863377609107,1.0,0.5502846299810247} 0.33$\pm$0.01 &                 \cellcolor[rgb]{0.963053912266994,1.0,0.5208170554749414} 0.19$\pm$0.01 & \cellcolor[rgb]{0.9384976001785912,1.0,0.5453733675633442} 0.28$\pm$0.02 \\
              Eccentricity Jaccard Score &                \cellcolor[rgb]{0.8981657179000632,1.0,0.5857052498418722} 0.18$\pm$0.02 &  \cellcolor[rgb]{0.9532313874316329,1.0,0.5306395803103024} 0.15$\pm$0.09 & \cellcolor[rgb]{0.8381887859508129,1.0,0.6456821817911225} 0.15$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.9421589986757232,0.5} 0.06$\pm$0.03 &                \cellcolor[rgb]{0.8381887859508129,1.0,0.6456821817911225} 0.42$\pm$0.01 &                 \cellcolor[rgb]{0.8431000483684934,1.0,0.640770919373442} 0.42$\pm$0.01 &                \cellcolor[rgb]{0.9935632697101611,0.9703532829253707,0.5} 0.19$\pm$0.04 &                \cellcolor[rgb]{0.8834319306470215,1.0,0.6004390370949139} 0.66$\pm$0.01 & \cellcolor[rgb]{0.8259106299066116,1.0,0.6579603378353239} 0.43$\pm$0.01 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.50$\pm$0.01 &                 \cellcolor[rgb]{0.8431000483684934,1.0,0.640770919373442} 0.41$\pm$0.01 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.46$\pm$0.02 \\
          Mahalanobis Distance - Decoder &                               \cellcolor[rgb]{1.0,0.6920842411038491,0.5} 0.00$\pm$0.01 &                \cellcolor[rgb]{1.0,0.6667093852791663,0.5} -0.01$\pm$0.10 &                \cellcolor[rgb]{1.0,0.8479217395019011,0.5} 0.00$\pm$0.03 &               \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.17$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.7101969328036227,0.5} -0.02$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8394634542270069,0.5} 0.06$\pm$0.01 &                \cellcolor[rgb]{0.9104438739442646,1.0,0.5734270937976709} 0.31$\pm$0.04 &                              \cellcolor[rgb]{1.0,0.8789354521765136,0.5} -0.30$\pm$0.03 &                 \cellcolor[rgb]{1.0,0.80161476355248,0.5} -0.07$\pm$0.01 &               \cellcolor[rgb]{1.0,0.8535605963518307,0.5} -0.10$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.7959759067025505,0.5} -0.14$\pm$0.01 &               \cellcolor[rgb]{1.0,0.8241701909521981,0.5} -0.21$\pm$0.03 \\
 Relative Mahalanobis Distance - Decoder &                               \cellcolor[rgb]{1.0,0.7553077876030589,0.5} 0.03$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.7959759067025505,0.5} 0.05$\pm$0.09 &               \cellcolor[rgb]{1.0,0.6526122431543425,0.5} -0.10$\pm$0.03 &              \cellcolor[rgb]{0.9999475726119325,0.5430817207057116,0.5} -0.24$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.6949036695288138,0.5} -0.04$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8344226579520698,0.5} 0.05$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.597846981930027,0.5} -0.25$\pm$0.03 & \cellcolor[rgb]{0.9679651746846745,0.9986330044000171,0.5159057930572609} 0.24$\pm$0.02 &                \cellcolor[rgb]{1.0,0.8591994532017602,0.5} 0.01$\pm$0.01 &                \cellcolor[rgb]{1.0,0.9393395702507584,0.5} 0.10$\pm$0.01 & \cellcolor[rgb]{0.9753320683111952,0.9912854030501093,0.5085388994307402} 0.17$\pm$0.01 &  \cellcolor[rgb]{0.9311307065520704,1.0,0.552740261189865} 0.30$\pm$0.02 \\
                           RDE - Decoder &                              \cellcolor[rgb]{1.0,0.5781109829552737,0.5} -0.05$\pm$0.01 &                \cellcolor[rgb]{1.0,0.5584604212055193,0.5} -0.06$\pm$0.10 &                \cellcolor[rgb]{1.0,0.9280618565508993,0.5} 0.04$\pm$0.03 &                \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.23$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.7214746465034817,0.5} -0.01$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8563800247767954,0.5} 0.08$\pm$0.01 &                \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.30$\pm$0.04 &                              \cellcolor[rgb]{1.0,0.8817548806014783,0.5} -0.29$\pm$0.03 &               \cellcolor[rgb]{1.0,0.8100730488273743,0.5} -0.06$\pm$0.01 &               \cellcolor[rgb]{1.0,0.8648383100516897,0.5} -0.08$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.8344226579520698,0.5} -0.08$\pm$0.01 &               \cellcolor[rgb]{1.0,0.8451023110769363,0.5} -0.15$\pm$0.03 \\
                        HUQ-MD - Decoder &                               \cellcolor[rgb]{1.0,0.8394634542270069,0.5} 0.07$\pm$0.01 &                \cellcolor[rgb]{1.0,0.6667093852791663,0.5} -0.01$\pm$0.10 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.13$\pm$0.03 &                             \cellcolor[rgb]{1.0,0.8072536204024094,0.5} -0.04$\pm$0.03 &                \cellcolor[rgb]{0.9409532313874316,1.0,0.5429177363545039} 0.30$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9337007134008288,0.5} 0.17$\pm$0.01 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.43$\pm$0.04 &                 \cellcolor[rgb]{0.8332775235331324,1.0,0.650593444208803} 0.93$\pm$0.00 & \cellcolor[rgb]{0.9655095434758343,1.0,0.5183614242661012} 0.21$\pm$0.01 &  \cellcolor[rgb]{0.990065855564237,0.9743688325003206,0.5} 0.19$\pm$0.01 &                \cellcolor[rgb]{0.9935632697101611,0.9703532829253707,0.5} 0.13$\pm$0.01 &                \cellcolor[rgb]{1.0,0.9365201418257938,0.5} 0.06$\pm$0.03 \\
                       HUQ-RMD - Decoder &                               \cellcolor[rgb]{1.0,0.9280618565508993,0.5} 0.11$\pm$0.02 &                 \cellcolor[rgb]{1.0,0.7734204793028324,0.5} 0.04$\pm$0.10 & \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.13$\pm$0.03 &                             \cellcolor[rgb]{1.0,0.8072536204024094,0.5} -0.04$\pm$0.03 &                \cellcolor[rgb]{0.9409532313874316,1.0,0.5429177363545039} 0.30$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9337007134008288,0.5} 0.17$\pm$0.01 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.43$\pm$0.03 &                 \cellcolor[rgb]{0.8332775235331324,1.0,0.650593444208803} 0.93$\pm$0.00 & \cellcolor[rgb]{0.9384976001785912,1.0,0.5453733675633442} 0.25$\pm$0.01 & \cellcolor[rgb]{0.9458644938051122,1.0,0.5380064739368233} 0.30$\pm$0.01 &                \cellcolor[rgb]{0.8736094058116604,1.0,0.6102615619302751} 0.35$\pm$0.01 & \cellcolor[rgb]{0.8883431930647021,1.0,0.5955277746772334} 0.42$\pm$0.02 \\
\bottomrule
\end{tabular}
}\caption{\label{tab:llama_2_results} PRR$\uparrow$ for the Llama v2 model with Rouge-L and BertScore as text quality metrics. Lighter color indicates better results.}\end{table*}

==> tables/camera_ready/vicuna.tex <==
\begin{table*}[!ht] \resizebox{\textwidth}{!}{\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{UE Method}} & \multicolumn{2}{c|}{\textbf{AESLC}} & \multicolumn{2}{c|}{\textbf{XSUM}} & \multicolumn{2}{c|}{\textbf{CoQA}} & \multicolumn{2}{c|}{\textbf{bAbiQA}} & \multicolumn{2}{c|}{\textbf{WMT14 De-En}} & \multicolumn{2}{c}{\textbf{WMT14 Fr-En}} \\ \cline{2-13}
    & \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore}&  \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore} \\\midrule
\midrule
            Maximum Sequence Probability &          \cellcolor[rgb]{0.9505975,0.9073195000000001,0.6585105} 0.24$\pm$0.01 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.19$\pm$0.10 &           \cellcolor[rgb]{0.6238025,0.648493,0.7114585} 0.01$\pm$0.03 &                \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.18$\pm$0.15 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.35$\pm$0.01 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.29$\pm$0.01 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.66$\pm$0.02 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.82$\pm$0.03 &                     \cellcolor[rgb]{0.880548,0.8501920000000001,0.706319} 0.32$\pm$0.01 &                      \cellcolor[rgb]{0.907637,0.872113,0.691252} 0.39$\pm$0.01 &            \cellcolor[rgb]{0.8702945,0.84195,0.7110655} 0.25$\pm$0.01 &          \cellcolor[rgb]{0.9034295,0.8686925,0.693842} 0.31$\pm$0.01 \\
                              Perplexity &           \cellcolor[rgb]{0.8621369999999999,0.8354295,0.714597} 0.19$\pm$0.01 &                    \cellcolor[rgb]{0.7258795,0.7269435,0.728791} 0.06$\pm$0.11 & \cellcolor[rgb]{0.7058035,0.7100725,0.7217884999999999} 0.04$\pm$0.03 & \cellcolor[rgb]{0.558806,0.6129675,0.7171540000000001} -0.13$\pm$0.13 &            \cellcolor[rgb]{0.7872085,0.776341,0.734586} 0.11$\pm$0.01 &                     \cellcolor[rgb]{0.727536,0.728359,0.729488} -0.09$\pm$0.02 &                             \cellcolor[rgb]{0.9976245,0.949192,0.6037805} 0.65$\pm$0.02 &                              \cellcolor[rgb]{0.9936465,0.942359,0.606668} 0.79$\pm$0.03 &                     \cellcolor[rgb]{0.972827,0.9256139999999999,0.635266} 0.41$\pm$0.01 &                     \cellcolor[rgb]{0.986557,0.936775,0.6173385} 0.47$\pm$0.01 &  \cellcolor[rgb]{0.963862,0.9182429999999999,0.6453055} 0.32$\pm$0.01 &         \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.35$\pm$0.01 \\
                      Mean Token Entropy &                      \cellcolor[rgb]{0.897149,0.863595,0.697508} 0.21$\pm$0.01 &            \cellcolor[rgb]{0.7626740000000001,0.7571425,0.73633} 0.08$\pm$0.11 &           \cellcolor[rgb]{0.730808,0.7312025,0.7309845} 0.05$\pm$0.03 &           \cellcolor[rgb]{0.5975285,0.632186,0.712962} -0.11$\pm$0.13 & \cellcolor[rgb]{0.7795905000000001,0.7703855,0.7354145} 0.10$\pm$0.01 & \cellcolor[rgb]{0.7159085000000001,0.718475,0.7249909999999999} -0.11$\pm$0.02 &          \cellcolor[rgb]{0.9182144999999999,0.8807415000000001,0.6843735} 0.52$\pm$0.02 &                   \cellcolor[rgb]{0.9505975,0.9073195000000001,0.6585105} 0.68$\pm$0.04 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.44$\pm$0.01 &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.49$\pm$0.01 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.35$\pm$0.01 &           \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.39$\pm$0.01 \\
            Pointwise Mutual Information &           \cellcolor[rgb]{0.5798665000000001,0.6226105,0.714764} 0.01$\pm$0.01 &                   \cellcolor[rgb]{0.5825565,0.6239825,0.714454} -0.01$\pm$0.11 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.14$\pm$0.03 &   \cellcolor[rgb]{0.816253,0.7990900000000001,0.729334} 0.06$\pm$0.13 &                \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.24$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.42$\pm$0.02 &                                \cellcolor[rgb]{0.71256,0.715667,0.723846} 0.14$\pm$0.03 &                             \cellcolor[rgb]{0.9013335,0.866989,0.6950765} 0.55$\pm$0.06 &           \cellcolor[rgb]{0.7159085000000001,0.718475,0.7249909999999999} 0.14$\pm$0.01 &           \cellcolor[rgb]{0.6548005,0.6701995000000001,0.712395} 0.09$\pm$0.01 &   \cellcolor[rgb]{0.707496,0.7114685000000001,0.722289} 0.11$\pm$0.01 &          \cellcolor[rgb]{0.6746705,0.685207,0.7148425} 0.10$\pm$0.01 \\
Conditional Pointwise Mutual Information &           \cellcolor[rgb]{0.8621369999999999,0.8354295,0.714597} 0.19$\pm$0.01 &                    \cellcolor[rgb]{0.7258795,0.7269435,0.728791} 0.06$\pm$0.11 & \cellcolor[rgb]{0.7058035,0.7100725,0.7217884999999999} 0.04$\pm$0.03 & \cellcolor[rgb]{0.558806,0.6129675,0.7171540000000001} -0.13$\pm$0.14 &            \cellcolor[rgb]{0.7872085,0.776341,0.734586} 0.11$\pm$0.01 &                     \cellcolor[rgb]{0.727536,0.728359,0.729488} -0.09$\pm$0.01 &                             \cellcolor[rgb]{0.9976245,0.949192,0.6037805} 0.65$\pm$0.02 &                              \cellcolor[rgb]{0.9936465,0.942359,0.606668} 0.79$\pm$0.03 &                     \cellcolor[rgb]{0.972827,0.9256139999999999,0.635266} 0.41$\pm$0.01 &                     \cellcolor[rgb]{0.986557,0.936775,0.6173385} 0.47$\pm$0.01 &  \cellcolor[rgb]{0.963862,0.9182429999999999,0.6453055} 0.32$\pm$0.01 &         \cellcolor[rgb]{0.9527945,0.9091285,0.6564445} 0.35$\pm$0.01 \\
                                 P(True) &                          \cellcolor[rgb]{0.5,0.589401,0.707382} -0.02$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.05$\pm$0.11 & \cellcolor[rgb]{0.9375285,0.8965624999999999,0.6698425} 0.12$\pm$0.03 &           \cellcolor[rgb]{0.975089,0.9274665,0.6325425} 0.17$\pm$0.13 &   \cellcolor[rgb]{0.7626740000000001,0.7571425,0.73633} 0.08$\pm$0.01 &                     \cellcolor[rgb]{0.850004,0.8257645,0.719312} 0.09$\pm$0.02 &                     \cellcolor[rgb]{0.792958,0.780837,0.7338089999999999} 0.30$\pm$0.03 &                             \cellcolor[rgb]{0.939689,0.8983435,0.6681205} 0.65$\pm$0.05 &                            \cellcolor[rgb]{0.585181,0.6253535,0.7141625} -0.00$\pm$0.01 &                             \cellcolor[rgb]{0.5,0.5854,0.69655} -0.05$\pm$0.01 &           \cellcolor[rgb]{0.6278655,0.6512045,0.711407} 0.04$\pm$0.01 &               \cellcolor[rgb]{0.5,0.590805,0.7109295} -0.02$\pm$0.01 \\
                        P(True) Sampling &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.04$\pm$0.01 &                          \cellcolor[rgb]{0.5,0.581529,0.685804} -0.04$\pm$0.11 &            \cellcolor[rgb]{0.905527,0.8704005,0.692599} 0.11$\pm$0.03 &          \cellcolor[rgb]{0.9289045,0.8894845,0.6766295} 0.14$\pm$0.13 &   \cellcolor[rgb]{0.8379905000000001,0.816234,0.723368} 0.17$\pm$0.01 & \cellcolor[rgb]{0.9182144999999999,0.8807415000000001,0.6843735} 0.18$\pm$0.02 &                            \cellcolor[rgb]{0.7515925,0.7484255,0.7361525} 0.22$\pm$0.03 &          \cellcolor[rgb]{0.9203465,0.8824810000000001,0.6828730000000001} 0.60$\pm$0.06 &                              \cellcolor[rgb]{0.5975285,0.632186,0.712962} 0.01$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.596683,0.7207805} -0.03$\pm$0.01 &            \cellcolor[rgb]{0.6154355,0.643067,0.711749} 0.03$\pm$0.01 &              \cellcolor[rgb]{0.5,0.5748955,0.6685325} -0.04$\pm$0.01 \\
            Monte Carlo Sequence Entropy &                    \cellcolor[rgb]{0.9139795,0.8772765,0.687146} 0.22$\pm$0.02 & \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.16$\pm$0.10 & \cellcolor[rgb]{0.6799580000000001,0.6893205,0.7157505} 0.03$\pm$0.03 & \cellcolor[rgb]{0.529189,0.6033145,0.7197655000000001} -0.14$\pm$0.15 &            \cellcolor[rgb]{0.986557,0.936775,0.6173385} 0.33$\pm$0.01 &          \cellcolor[rgb]{0.9819359999999999,0.9330445,0.6237225} 0.26$\pm$0.01 &                             \cellcolor[rgb]{0.9976245,0.949192,0.6037805} 0.65$\pm$0.02 &                    \cellcolor[rgb]{0.9974235,0.946477,0.6017224999999999} 0.80$\pm$0.03 &                     \cellcolor[rgb]{0.880548,0.8501920000000001,0.706319} 0.32$\pm$0.01 &                      \cellcolor[rgb]{0.907637,0.872113,0.691252} 0.39$\pm$0.01 &            \cellcolor[rgb]{0.8702945,0.84195,0.7110655} 0.25$\pm$0.01 &          \cellcolor[rgb]{0.9034295,0.8686925,0.693842} 0.31$\pm$0.01 \\
 Monte Carlo Normalized Sequence Entropy & \cellcolor[rgb]{0.8459855000000001,0.8225724999999999,0.7207455} 0.18$\pm$0.01 &                    \cellcolor[rgb]{0.7258795,0.7269435,0.728791} 0.06$\pm$0.10 &    \cellcolor[rgb]{0.7571129999999999,0.752773,0.73632} 0.06$\pm$0.03 &               \cellcolor[rgb]{0.5,0.5943845,0.7197815} -0.15$\pm$0.13 &  \cellcolor[rgb]{0.7720345,0.764474,0.7359735000000001} 0.09$\pm$0.01 &                    \cellcolor[rgb]{0.722574,0.724113,0.7274425} -0.10$\pm$0.01 &                             \cellcolor[rgb]{0.979642,0.9311825,0.6267815} 0.62$\pm$0.02 &                   \cellcolor[rgb]{0.9505975,0.9073195000000001,0.6585105} 0.68$\pm$0.03 &                     \cellcolor[rgb]{0.972827,0.9256139999999999,0.635266} 0.41$\pm$0.01 &                     \cellcolor[rgb]{0.986557,0.936775,0.6173385} 0.47$\pm$0.01 & \cellcolor[rgb]{0.9505975,0.9073195000000001,0.6585105} 0.31$\pm$0.01 &          \cellcolor[rgb]{0.939689,0.8983435,0.6681205} 0.34$\pm$0.01 \\
                        Semantic Entropy &                    \cellcolor[rgb]{0.9139795,0.8772765,0.687146} 0.22$\pm$0.01 & \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.16$\pm$0.10 & \cellcolor[rgb]{0.7058035,0.7100725,0.7217884999999999} 0.04$\pm$0.03 &           \cellcolor[rgb]{0.5975285,0.632186,0.712962} -0.11$\pm$0.14 &           \cellcolor[rgb]{0.975089,0.9274665,0.6325425} 0.32$\pm$0.01 &            \cellcolor[rgb]{0.972827,0.9256139999999999,0.635266} 0.25$\pm$0.01 &                             \cellcolor[rgb]{0.9976245,0.949192,0.6037805} 0.65$\pm$0.02 &                              \cellcolor[rgb]{0.9936465,0.942359,0.606668} 0.79$\pm$0.03 &                     \cellcolor[rgb]{0.880548,0.8501920000000001,0.706319} 0.32$\pm$0.01 &                      \cellcolor[rgb]{0.907637,0.872113,0.691252} 0.39$\pm$0.01 &            \cellcolor[rgb]{0.8702945,0.84195,0.7110655} 0.25$\pm$0.01 &          \cellcolor[rgb]{0.9034295,0.8686925,0.693842} 0.31$\pm$0.01 \\
              Lexical Similarity Rouge-1 &                      \cellcolor[rgb]{0.830041,0.809952,0.725767} 0.17$\pm$0.01 &          \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.15$\pm$0.11 &            \cellcolor[rgb]{0.814288,0.797552,0.7298205} 0.08$\pm$0.03 &              \cellcolor[rgb]{0.749776,0.74698,0.736016} 0.01$\pm$0.13 &   \cellcolor[rgb]{0.8379905000000001,0.816234,0.723368} 0.17$\pm$0.01 &            \cellcolor[rgb]{0.880548,0.8501920000000001,0.706319} 0.13$\pm$0.02 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.43$\pm$0.03 &                   \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.58$\pm$0.04 &                     \cellcolor[rgb]{0.8221350000000001,0.803725,0.727943} 0.26$\pm$0.01 &  \cellcolor[rgb]{0.8064884999999999,0.7914304999999999,0.731475} 0.28$\pm$0.01 &            \cellcolor[rgb]{0.737406,0.736916,0.7338405} 0.14$\pm$0.01 &           \cellcolor[rgb]{0.704113,0.7086785,0.721285} 0.13$\pm$0.01 \\
              Lexical Similarity Rouge-2 &                      \cellcolor[rgb]{0.830041,0.809952,0.725767} 0.17$\pm$0.01 &            \cellcolor[rgb]{0.868244,0.8403145000000001,0.712014} 0.13$\pm$0.10 &            \cellcolor[rgb]{0.814288,0.797552,0.7298205} 0.08$\pm$0.03 &          \cellcolor[rgb]{0.7258795,0.7269435,0.728791} -0.01$\pm$0.15 &           \cellcolor[rgb]{0.7258795,0.7269435,0.728791} 0.03$\pm$0.01 &                    \cellcolor[rgb]{0.722574,0.724113,0.7274425} -0.10$\pm$0.01 &                              \cellcolor[rgb]{0.652943,0.6688405,0.712256} 0.02$\pm$0.03 &                                  \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.64$\pm$0.07 &                     \cellcolor[rgb]{0.8221350000000001,0.803725,0.727943} 0.26$\pm$0.01 &            \cellcolor[rgb]{0.816253,0.7990900000000001,0.729334} 0.29$\pm$0.01 &            \cellcolor[rgb]{0.737406,0.736916,0.7338405} 0.14$\pm$0.01 &          \cellcolor[rgb]{0.7242235,0.7255265,0.728132} 0.15$\pm$0.01 \\
              Lexical Similarity Rouge-L &                      \cellcolor[rgb]{0.830041,0.809952,0.725767} 0.17$\pm$0.02 &          \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.15$\pm$0.11 &  \cellcolor[rgb]{0.8439785,0.820983,0.7214430000000001} 0.09$\pm$0.03 &            \cellcolor[rgb]{0.737406,0.736916,0.7338405} 0.00$\pm$0.13 &   \cellcolor[rgb]{0.8379905000000001,0.816234,0.723368} 0.17$\pm$0.01 &            \cellcolor[rgb]{0.880548,0.8501920000000001,0.706319} 0.13$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.43$\pm$0.03 &                   \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.58$\pm$0.04 &                              \cellcolor[rgb]{0.812327,0.796017,0.7302915} 0.25$\pm$0.01 &  \cellcolor[rgb]{0.8064884999999999,0.7914304999999999,0.731475} 0.28$\pm$0.01 &            \cellcolor[rgb]{0.737406,0.736916,0.7338405} 0.14$\pm$0.01 &          \cellcolor[rgb]{0.7242235,0.7255265,0.728132} 0.15$\pm$0.01 \\
                 Lexical Similarity BLEU &                   \cellcolor[rgb]{0.7664145,0.7600675,0.7362005} 0.13$\pm$0.01 &            \cellcolor[rgb]{0.7626740000000001,0.7571425,0.73633} 0.08$\pm$0.11 &            \cellcolor[rgb]{0.814288,0.797552,0.7298205} 0.08$\pm$0.03 &   \cellcolor[rgb]{0.7142310000000001,0.71707,0.724432} -0.02$\pm$0.13 &            \cellcolor[rgb]{0.812327,0.796017,0.7302915} 0.14$\pm$0.01 &                     \cellcolor[rgb]{0.8580885,0.832192,0.716193} 0.10$\pm$0.02 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.43$\pm$0.03 &                              \cellcolor[rgb]{0.905527,0.8704005,0.692599} 0.56$\pm$0.05 &                     \cellcolor[rgb]{0.792958,0.780837,0.7338089999999999} 0.23$\pm$0.01 &                     \cellcolor[rgb]{0.834004,0.8130855,0.724635} 0.31$\pm$0.01 &             \cellcolor[rgb]{0.727536,0.728359,0.729488} 0.13$\pm$0.01 & \cellcolor[rgb]{0.734127,0.7340415,0.7324539999999999} 0.16$\pm$0.01 \\
                              NumSemSets &                   \cellcolor[rgb]{0.7515925,0.7484255,0.7361525} 0.12$\pm$0.01 & \cellcolor[rgb]{0.8459855000000001,0.8225724999999999,0.7207455} 0.12$\pm$0.11 & \cellcolor[rgb]{0.7058035,0.7100725,0.7217884999999999} 0.04$\pm$0.03 &   \cellcolor[rgb]{0.828057,0.8083899999999999,0.726351} 0.07$\pm$0.15 & \cellcolor[rgb]{0.7968109999999999,0.7838485,0.7332005} 0.12$\pm$0.01 &           \cellcolor[rgb]{0.8439785,0.820983,0.7214430000000001} 0.08$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.43$\pm$0.03 &                              \cellcolor[rgb]{0.916096,0.879007,0.6857645} 0.59$\pm$0.05 &                                \cellcolor[rgb]{0.61756,0.644424,0.711652} 0.03$\pm$0.01 &                     \cellcolor[rgb]{0.645442,0.663408,0.7117585} 0.08$\pm$0.01 &       \cellcolor[rgb]{0.5,0.592275,0.7144010000000001} -0.03$\pm$0.01 &          \cellcolor[rgb]{0.539312,0.606061,0.7190525} -0.00$\pm$0.01 \\
       EigValLaplacian NLI Score entail. &                     \cellcolor[rgb]{0.814288,0.797552,0.7298205} 0.16$\pm$0.01 & \cellcolor[rgb]{0.8459855000000001,0.8225724999999999,0.7207455} 0.12$\pm$0.11 & \cellcolor[rgb]{0.7853034999999999,0.7748475,0.7347965} 0.07$\pm$0.03 &   \cellcolor[rgb]{0.7626740000000001,0.7571425,0.73633} 0.02$\pm$0.13 &            \cellcolor[rgb]{0.864167,0.8370535,0.713777} 0.20$\pm$0.01 &                    \cellcolor[rgb]{0.9034295,0.8686925,0.693842} 0.16$\pm$0.01 &                              \cellcolor[rgb]{0.8045525,0.789908,0.731819} 0.32$\pm$0.03 &                    \cellcolor[rgb]{0.895058,0.8619049999999999,0.6987115} 0.53$\pm$0.05 &                             \cellcolor[rgb]{0.7479565,0.745538,0.7358755} 0.18$\pm$0.01 &           \cellcolor[rgb]{0.7720345,0.764474,0.7359735000000001} 0.24$\pm$0.01 &   \cellcolor[rgb]{0.717584,0.7198815000000001,0.725567} 0.12$\pm$0.01 &   \cellcolor[rgb]{0.7142310000000001,0.71707,0.724432} 0.14$\pm$0.01 \\
       EigValLaplacian NLI Score Contra. &                   \cellcolor[rgb]{0.7664145,0.7600675,0.7362005} 0.13$\pm$0.01 &            \cellcolor[rgb]{0.868244,0.8403145000000001,0.712014} 0.13$\pm$0.11 &    \cellcolor[rgb]{0.7571129999999999,0.752773,0.73632} 0.06$\pm$0.03 &            \cellcolor[rgb]{0.789118,0.7778365,0.734362} 0.04$\pm$0.13 &   \cellcolor[rgb]{0.8479924999999999,0.824167,0.720036} 0.18$\pm$0.01 &            \cellcolor[rgb]{0.880548,0.8501920000000001,0.706319} 0.13$\pm$0.02 &                    \cellcolor[rgb]{0.820176,0.8021769999999999,0.7283955} 0.35$\pm$0.03 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.45$\pm$0.05 &                      \cellcolor[rgb]{0.7571129999999999,0.752773,0.73632} 0.19$\pm$0.01 &            \cellcolor[rgb]{0.816253,0.7990900000000001,0.729334} 0.29$\pm$0.01 &             \cellcolor[rgb]{0.685215,0.693445,0.716714} 0.09$\pm$0.01 &           \cellcolor[rgb]{0.704113,0.7086785,0.721285} 0.13$\pm$0.01 \\
           EigValLaplacian Jaccard Score &                   \cellcolor[rgb]{0.7664145,0.7600675,0.7362005} 0.13$\pm$0.01 &                    \cellcolor[rgb]{0.824111,0.8052765,0.7274005} 0.11$\pm$0.11 &  \cellcolor[rgb]{0.8439785,0.820983,0.7214430000000001} 0.09$\pm$0.03 &           \cellcolor[rgb]{0.737406,0.736916,0.7338405} -0.00$\pm$0.13 &            \cellcolor[rgb]{0.812327,0.796017,0.7302915} 0.14$\pm$0.01 &                     \cellcolor[rgb]{0.850004,0.8257645,0.719312} 0.09$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.43$\pm$0.03 &                              \cellcolor[rgb]{0.916096,0.879007,0.6857645} 0.59$\pm$0.04 & \cellcolor[rgb]{0.8026055000000001,0.7883884999999999,0.7322204999999999} 0.24$\pm$0.01 &                     \cellcolor[rgb]{0.834004,0.8130855,0.724635} 0.31$\pm$0.01 &            \cellcolor[rgb]{0.737406,0.736916,0.7338405} 0.14$\pm$0.01 & \cellcolor[rgb]{0.7443485,0.742659,0.7355039999999999} 0.17$\pm$0.01 \\
                DegMat NLI Score entail. &                     \cellcolor[rgb]{0.814288,0.797552,0.7298205} 0.16$\pm$0.02 &          \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.15$\pm$0.11 &            \cellcolor[rgb]{0.814288,0.797552,0.7298205} 0.08$\pm$0.03 &   \cellcolor[rgb]{0.816253,0.7990900000000001,0.729334} 0.06$\pm$0.13 &            \cellcolor[rgb]{0.812327,0.796017,0.7302915} 0.14$\pm$0.01 &                      \cellcolor[rgb]{0.830041,0.809952,0.725767} 0.06$\pm$0.01 &                             \cellcolor[rgb]{0.8888255,0.8568595,0.702056} 0.47$\pm$0.03 &                             \cellcolor[rgb]{0.9013335,0.866989,0.6950765} 0.55$\pm$0.05 &                             \cellcolor[rgb]{0.739093,0.7383495,0.7344225} 0.17$\pm$0.01 & \cellcolor[rgb]{0.8419749999999999,0.8193965000000001,0.7221255} 0.32$\pm$0.01 &   \cellcolor[rgb]{0.783401,0.7733574999999999,0.734994} 0.18$\pm$0.01 &           \cellcolor[rgb]{0.8560525,0.83058,0.7170585} 0.27$\pm$0.01 \\
                DegMat NLI Score Contra. &                   \cellcolor[rgb]{0.7515925,0.7484255,0.7361525} 0.12$\pm$0.01 &                     \cellcolor[rgb]{0.8045525,0.789908,0.731819} 0.10$\pm$0.11 &           \cellcolor[rgb]{0.9705735,0.923765,0.6379075} 0.13$\pm$0.03 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.19$\pm$0.13 &          \cellcolor[rgb]{0.7324735,0.7326205,0.7316975} 0.04$\pm$0.01 &                   \cellcolor[rgb]{0.740811,0.7397865,0.7348835} -0.07$\pm$0.01 &          \cellcolor[rgb]{0.9182144999999999,0.8807415000000001,0.6843735} 0.52$\pm$0.02 &                              \cellcolor[rgb]{0.8908975,0.858537,0.700983} 0.52$\pm$0.04 &                             \cellcolor[rgb]{0.7479565,0.745538,0.7358755} 0.18$\pm$0.01 &                   \cellcolor[rgb]{0.8520185,0.8273655,0.7185735} 0.33$\pm$0.01 &             \cellcolor[rgb]{0.727536,0.728359,0.729488} 0.13$\pm$0.01 &  \cellcolor[rgb]{0.8320274999999999,0.811517,0.725169} 0.25$\pm$0.01 \\
                    DegMat Jaccard Score &                   \cellcolor[rgb]{0.7664145,0.7600675,0.7362005} 0.13$\pm$0.02 &                    \cellcolor[rgb]{0.824111,0.8052765,0.7274005} 0.11$\pm$0.11 &            \cellcolor[rgb]{0.814288,0.797552,0.7298205} 0.08$\pm$0.03 &           \cellcolor[rgb]{0.737406,0.736916,0.7338405} -0.00$\pm$0.13 &   \cellcolor[rgb]{0.8221350000000001,0.803725,0.727943} 0.15$\pm$0.01 &                     \cellcolor[rgb]{0.850004,0.8257645,0.719312} 0.09$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.43$\pm$0.03 &                   \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.58$\pm$0.05 &                     \cellcolor[rgb]{0.783401,0.7733574999999999,0.734994} 0.22$\pm$0.01 &                    \cellcolor[rgb]{0.824111,0.8052765,0.7274005} 0.30$\pm$0.01 &            \cellcolor[rgb]{0.737406,0.736916,0.7338405} 0.14$\pm$0.01 &          \cellcolor[rgb]{0.7242235,0.7255265,0.728132} 0.15$\pm$0.01 \\
          Eccentricity NLI Score entail. &                     \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.27$\pm$0.01 &          \cellcolor[rgb]{0.9819359999999999,0.9330445,0.6237225} 0.18$\pm$0.11 & \cellcolor[rgb]{0.7058035,0.7100725,0.7217884999999999} 0.04$\pm$0.03 &   \cellcolor[rgb]{0.7142310000000001,0.71707,0.724432} -0.02$\pm$0.13 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.35$\pm$0.01 &          \cellcolor[rgb]{0.9819359999999999,0.9330445,0.6237225} 0.26$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.43$\pm$0.02 &                    \cellcolor[rgb]{0.9310525000000001,0.891247,0.6750055} 0.63$\pm$0.04 &                               \cellcolor[rgb]{0.830041,0.809952,0.725767} 0.27$\pm$0.01 &                      \cellcolor[rgb]{0.897149,0.863595,0.697508} 0.38$\pm$0.01 &   \cellcolor[rgb]{0.783401,0.7733574999999999,0.734994} 0.18$\pm$0.01 & \cellcolor[rgb]{0.820176,0.8021769999999999,0.7283955} 0.24$\pm$0.01 \\
          Eccentricity NLI Score Contra. &                      \cellcolor[rgb]{0.897149,0.863595,0.697508} 0.21$\pm$0.01 & \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.16$\pm$0.11 & \cellcolor[rgb]{0.7853034999999999,0.7748475,0.7347965} 0.07$\pm$0.03 &  \cellcolor[rgb]{0.9440405000000001,0.9019195,0.664385} 0.15$\pm$0.14 &            \cellcolor[rgb]{0.8560525,0.83058,0.7170585} 0.19$\pm$0.01 &            \cellcolor[rgb]{0.8221350000000001,0.803725,0.727943} 0.05$\pm$0.01 &                            \cellcolor[rgb]{0.8826115,0.8518525,0.7052935} 0.46$\pm$0.03 &                   \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.58$\pm$0.05 &                    \cellcolor[rgb]{0.7739199999999999,0.7659475,0.735852} 0.21$\pm$0.01 &  \cellcolor[rgb]{0.8601110000000001,0.833809,0.7154024999999999} 0.34$\pm$0.01 &          \cellcolor[rgb]{0.7608215,0.7556835,0.7363195} 0.16$\pm$0.01 & \cellcolor[rgb]{0.8439785,0.820983,0.7214430000000001} 0.26$\pm$0.01 \\
              Eccentricity Jaccard Score &           \cellcolor[rgb]{0.9310525000000001,0.891247,0.6750055} 0.23$\pm$0.01 &            \cellcolor[rgb]{0.868244,0.8403145000000001,0.712014} 0.13$\pm$0.10 & \cellcolor[rgb]{0.7853034999999999,0.7748475,0.7347965} 0.07$\pm$0.03 &          \cellcolor[rgb]{0.6675365,0.679737,0.7138025} -0.06$\pm$0.13 &   \cellcolor[rgb]{0.9462200000000001,0.903715,0.662484} 0.29$\pm$0.01 &          \cellcolor[rgb]{0.9246114999999999,0.8859735,0.6798645} 0.19$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.43$\pm$0.03 &          \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.64$\pm$0.05 &                            \cellcolor[rgb]{0.9097495,0.8738295,0.6898925} 0.35$\pm$0.01 & \cellcolor[rgb]{0.9353585,0.8947860000000001,0.6716664999999999} 0.42$\pm$0.01 &             \cellcolor[rgb]{0.897149,0.863595,0.697508} 0.27$\pm$0.01 &           \cellcolor[rgb]{0.916096,0.879007,0.6857645} 0.32$\pm$0.01 \\
          Mahalanobis Distance - Decoder &                       \cellcolor[rgb]{0.61756,0.644424,0.711652} 0.03$\pm$0.01 &                   \cellcolor[rgb]{0.5825565,0.6239825,0.714454} -0.01$\pm$0.11 & \cellcolor[rgb]{0.6799580000000001,0.6893205,0.7157505} 0.03$\pm$0.03 &           \cellcolor[rgb]{0.775806,0.7674245,0.7357195} 0.03$\pm$0.15 &           \cellcolor[rgb]{0.7258795,0.7269435,0.728791} 0.03$\pm$0.01 &                     \cellcolor[rgb]{0.8359955,0.814658,0.724009} 0.07$\pm$0.01 &                    \cellcolor[rgb]{0.8260890000000001,0.806832,0.7268445} 0.36$\pm$0.03 &                            \cellcolor[rgb]{0.9097495,0.8738295,0.6898925} 0.57$\pm$0.05 &                             \cellcolor[rgb]{0.555329,0.611585,0.7175335} -0.02$\pm$0.01 &                  \cellcolor[rgb]{0.5621455,0.6143485,0.7167735} -0.00$\pm$0.01 &  \cellcolor[rgb]{0.508926,0.599264,0.7206239999999999} -0.02$\pm$0.01 &          \cellcolor[rgb]{0.501801,0.5979555,0.720782} -0.01$\pm$0.01 \\
 Relative Mahalanobis Distance - Decoder &                    \cellcolor[rgb]{0.599882,0.6335495,0.7127485} 0.02$\pm$0.01 &                     \cellcolor[rgb]{0.690415,0.697582,0.7178265} 0.04$\pm$0.11 &                \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.03$\pm$0.03 & \cellcolor[rgb]{0.6548005,0.6701995000000001,0.712395} -0.07$\pm$0.12 &           \cellcolor[rgb]{0.7258795,0.7269435,0.728791} 0.03$\pm$0.01 &                     \cellcolor[rgb]{0.8359955,0.814658,0.724009} 0.07$\pm$0.02 &                                  \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.25$\pm$0.04 &                              \cellcolor[rgb]{0.729183,0.729776,0.7302285} 0.04$\pm$0.08 &                                  \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.09$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.08$\pm$0.01 &                \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.06$\pm$0.01 &               \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.05$\pm$0.01 \\
                           RDE - Decoder &                         \cellcolor[rgb]{0.5,0.578966,0.6787605} -0.03$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} -0.05$\pm$0.11 & \cellcolor[rgb]{0.7853034999999999,0.7748475,0.7347965} 0.07$\pm$0.03 &            \cellcolor[rgb]{0.8560525,0.83058,0.7170585} 0.09$\pm$0.13 &          \cellcolor[rgb]{0.7324735,0.7326205,0.7316975} 0.04$\pm$0.01 &                     \cellcolor[rgb]{0.850004,0.8257645,0.719312} 0.09$\pm$0.02 &                              \cellcolor[rgb]{0.7872085,0.776341,0.734586} 0.29$\pm$0.03 &                             \cellcolor[rgb]{0.8540335,0.828971,0.7178235} 0.42$\pm$0.06 &                    \cellcolor[rgb]{0.571426,0.618486,0.7157020000000001} -0.01$\pm$0.01 &                   \cellcolor[rgb]{0.5231025,0.6019515,0.720098} -0.02$\pm$0.01 &         \cellcolor[rgb]{0.5478225,0.6088215,0.7182965} -0.01$\pm$0.01 &               \cellcolor[rgb]{0.5,0.590805,0.7109295} -0.02$\pm$0.01 \\
                        HUQ-MD - Decoder &           \cellcolor[rgb]{0.8621369999999999,0.8354295,0.714597} 0.19$\pm$0.01 &                    \cellcolor[rgb]{0.7258795,0.7269435,0.728791} 0.06$\pm$0.11 & \cellcolor[rgb]{0.6799580000000001,0.6893205,0.7157505} 0.03$\pm$0.03 &  \cellcolor[rgb]{0.613299,0.6417094999999999,0.711839} -0.10$\pm$0.14 &  \cellcolor[rgb]{0.7720345,0.764474,0.7359735000000001} 0.09$\pm$0.01 &                  \cellcolor[rgb]{0.7664145,0.7600675,0.7362005} -0.03$\pm$0.02 &                             \cellcolor[rgb]{0.979642,0.9311825,0.6267815} 0.62$\pm$0.02 &                   \cellcolor[rgb]{0.9819359999999999,0.9330445,0.6237225} 0.76$\pm$0.03 &                              \cellcolor[rgb]{0.850004,0.8257645,0.719312} 0.29$\pm$0.01 &          \cellcolor[rgb]{0.8784875,0.8485355,0.7073294999999999} 0.36$\pm$0.01 &   \cellcolor[rgb]{0.8320274999999999,0.811517,0.725169} 0.22$\pm$0.01 & \cellcolor[rgb]{0.8439785,0.820983,0.7214430000000001} 0.26$\pm$0.01 \\
                       HUQ-RMD - Decoder &           \cellcolor[rgb]{0.8621369999999999,0.8354295,0.714597} 0.19$\pm$0.01 &                    \cellcolor[rgb]{0.7258795,0.7269435,0.728791} 0.06$\pm$0.11 &            \cellcolor[rgb]{0.652943,0.6688405,0.712256} 0.02$\pm$0.03 & \cellcolor[rgb]{0.558806,0.6129675,0.7171540000000001} -0.13$\pm$0.14 &  \cellcolor[rgb]{0.7720345,0.764474,0.7359735000000001} 0.09$\pm$0.01 &                  \cellcolor[rgb]{0.7664145,0.7600675,0.7362005} -0.03$\pm$0.01 &                   \cellcolor[rgb]{0.7987345,0.7853589999999999,0.7329105} 0.31$\pm$0.03 &          \cellcolor[rgb]{0.9203465,0.8824810000000001,0.6828730000000001} 0.60$\pm$0.05 &                     \cellcolor[rgb]{0.783401,0.7733574999999999,0.734994} 0.22$\pm$0.01 &                     \cellcolor[rgb]{0.789118,0.7778365,0.734362} 0.26$\pm$0.01 & \cellcolor[rgb]{0.7968109999999999,0.7838485,0.7332005} 0.19$\pm$0.01 &           \cellcolor[rgb]{0.7872085,0.776341,0.734586} 0.21$\pm$0.01 \\
\bottomrule
\end{tabular}
}\caption{\label{tab:vicuna_results} PRR$\uparrow$ for the Vicuna model with Rouge-L and BertScore as text quality metrics. Lighter color indicates better results.}\end{table*}

==> tables/camera_ready/vicuna_red_green.tex <==
\begin{table*}[!ht] \resizebox{\textwidth}{!}{\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{UE Method}} & \multicolumn{2}{c|}{\textbf{AESLC}} & \multicolumn{2}{c|}{\textbf{XSUM}} & \multicolumn{2}{c|}{\textbf{CoQA}} & \multicolumn{2}{c|}{\textbf{bAbiQA}} & \multicolumn{2}{c|}{\textbf{WMT14 De-En}} & \multicolumn{2}{c}{\textbf{WMT14 Fr-En}} \\ \cline{2-13}
    & \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore}&  \textbf{Rouge-L} & \textbf{BERTScore}& \textbf{Rouge-L} & \textbf{BERTScore} \\\midrule
\midrule
            Maximum Sequence Probability &                \cellcolor[rgb]{0.8736094058116604,1.0,0.6102615619302751} 0.24$\pm$0.01 &   \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.19$\pm$0.10 &                \cellcolor[rgb]{1.0,0.6695288137041311,0.5} 0.01$\pm$0.03 &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.18$\pm$0.15 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.35$\pm$0.01 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.29$\pm$0.01 &  \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.66$\pm$0.02 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.82$\pm$0.03 &                 \cellcolor[rgb]{0.9483201250139524,1.0,0.535550842727983} 0.32$\pm$0.01 &                \cellcolor[rgb]{0.9227220299884659,1.0,0.5611489377534695} 0.39$\pm$0.01 & \cellcolor[rgb]{0.9605982810581537,1.0,0.5232726866837817} 0.25$\pm$0.01 &                \cellcolor[rgb]{0.9276332924061464,1.0,0.5562376753357889} 0.31$\pm$0.01 \\
                              Perplexity & \cellcolor[rgb]{0.9704208058935146,0.9963774616600456,0.5134501618484207} 0.19$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.8157119056773038,0.5} 0.06$\pm$0.11 &                \cellcolor[rgb]{1.0,0.7818787645777266,0.5} 0.04$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.6034858387799565,0.5} -0.13$\pm$0.13 &                               \cellcolor[rgb]{1.0,0.8997821350762528,0.5} 0.11$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.8185313341022685,0.5} -0.09$\pm$0.02 & \cellcolor[rgb]{0.8259106299066116,1.0,0.6579603378353239} 0.65$\pm$0.02 &                 \cellcolor[rgb]{0.8332775235331324,1.0,0.650593444208803} 0.79$\pm$0.03 &                \cellcolor[rgb]{0.8553782044126947,1.0,0.6284927633292406} 0.41$\pm$0.01 &                \cellcolor[rgb]{0.8406444171596532,1.0,0.6432265505822823} 0.47$\pm$0.01 & \cellcolor[rgb]{0.8652007292480559,1.0,0.6186702384938796} 0.32$\pm$0.01 &                \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.35$\pm$0.01 \\
                      Mean Token Entropy &                \cellcolor[rgb]{0.9286750753432302,1.0,0.5551958923987053} 0.21$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.8676577384766544,0.5} 0.08$\pm$0.11 &                \cellcolor[rgb]{1.0,0.8241701909521981,0.5} 0.05$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.635695672604554,0.5} -0.11$\pm$0.13 &                               \cellcolor[rgb]{1.0,0.8930325943013373,0.5} 0.10$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.7987953351275152,0.5} -0.11$\pm$0.02 & \cellcolor[rgb]{0.9104438739442646,1.0,0.5734270937976709} 0.52$\pm$0.02 &                \cellcolor[rgb]{0.8736094058116604,1.0,0.6102615619302751} 0.68$\pm$0.04 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.44$\pm$0.01 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.49$\pm$0.01 &  \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.35$\pm$0.01 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.39$\pm$0.01 \\
            Pointwise Mutual Information &                               \cellcolor[rgb]{1.0,0.6232218377547099,0.5} 0.01$\pm$0.01 &                \cellcolor[rgb]{1.0,0.6238198983297023,0.5} -0.01$\pm$0.11 &  \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.14$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.9393395702507584,0.5} 0.06$\pm$0.13 &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.24$\pm$0.01 &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.42$\pm$0.02 &                \cellcolor[rgb]{1.0,0.7931564782775857,0.5} 0.14$\pm$0.03 &                \cellcolor[rgb]{0.9285262492093611,1.0,0.5553447185325744} 0.55$\pm$0.06 &                               \cellcolor[rgb]{1.0,0.7987953351275152,0.5} 0.14$\pm$0.01 &                                \cellcolor[rgb]{1.0,0.707377504378658,0.5} 0.09$\pm$0.01 &                \cellcolor[rgb]{1.0,0.7846981930026914,0.5} 0.11$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.7383912170532703,0.5} 0.10$\pm$0.01 \\
Conditional Pointwise Mutual Information & \cellcolor[rgb]{0.9704208058935146,0.9963774616600456,0.5134501618484207} 0.19$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.8157119056773038,0.5} 0.06$\pm$0.11 &                \cellcolor[rgb]{1.0,0.7818787645777266,0.5} 0.04$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.6034858387799565,0.5} -0.13$\pm$0.14 &                               \cellcolor[rgb]{1.0,0.8997821350762528,0.5} 0.11$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.8185313341022685,0.5} -0.09$\pm$0.01 & \cellcolor[rgb]{0.8259106299066116,1.0,0.6579603378353239} 0.65$\pm$0.02 &                 \cellcolor[rgb]{0.8332775235331324,1.0,0.650593444208803} 0.79$\pm$0.03 &                \cellcolor[rgb]{0.8553782044126947,1.0,0.6284927633292406} 0.41$\pm$0.01 &                \cellcolor[rgb]{0.8406444171596532,1.0,0.6432265505822823} 0.47$\pm$0.01 & \cellcolor[rgb]{0.8652007292480559,1.0,0.6186702384938796} 0.32$\pm$0.01 &                \cellcolor[rgb]{0.8716002530044273,1.0,0.6122707147375082} 0.35$\pm$0.01 \\
                                 P(True) &                              \cellcolor[rgb]{1.0,0.5584604212055193,0.5} -0.02$\pm$0.01 &  \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.05$\pm$0.11 & \cellcolor[rgb]{0.8883431930647021,1.0,0.5955277746772334} 0.12$\pm$0.03 &                \cellcolor[rgb]{0.8529225732038546,1.0,0.6309483945380809} 0.17$\pm$0.13 &                               \cellcolor[rgb]{1.0,0.8676577384766544,0.5} 0.08$\pm$0.01 & \cellcolor[rgb]{0.9851545931465564,0.9800076893502501,0.5002232392008037} 0.09$\pm$0.02 &                \cellcolor[rgb]{1.0,0.9055064291511813,0.5} 0.30$\pm$0.03 &                \cellcolor[rgb]{0.8858875618558619,1.0,0.5979834058860736} 0.65$\pm$0.05 &                              \cellcolor[rgb]{1.0,0.6238198983297023,0.5} -0.00$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.5515400059806059,0.5} -0.05$\pm$0.01 &                \cellcolor[rgb]{1.0,0.6751676705540606,0.5} 0.04$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.5584604212055193,0.5} -0.02$\pm$0.01 \\
                        %P(True) Sampling &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.04$\pm$0.01 & \cellcolor[rgb]{0.9999475726119325,0.5430817207057116,0.5} -0.04$\pm$0.11 & \cellcolor[rgb]{0.9251776611973062,1.0,0.5586933065446292} 0.11$\pm$0.03 &                \cellcolor[rgb]{0.8981657179000632,1.0,0.5857052498418722} 0.14$\pm$0.13 &                \cellcolor[rgb]{0.9935632697101611,0.9703532829253707,0.5} 0.17$\pm$0.01 &                \cellcolor[rgb]{0.9104438739442646,1.0,0.5734270937976709} 0.18$\pm$0.02 &                \cellcolor[rgb]{1.0,0.8507411679268658,0.5} 0.22$\pm$0.03 &                \cellcolor[rgb]{0.9079882427354242,1.0,0.5758827250065112} 0.60$\pm$0.06 &                                \cellcolor[rgb]{1.0,0.635695672604554,0.5} 0.01$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.5696526976803795,0.5} -0.03$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.658251100004272,0.5} 0.03$\pm$0.01 &                \cellcolor[rgb]{0.9901174373492717,0.528984578580888,0.5} -0.04$\pm$0.01 \\
            Monte Carlo Sequence Entropy &                \cellcolor[rgb]{0.9153551363619451,1.0,0.5685158313799904} 0.22$\pm$0.02 &  \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.16$\pm$0.10 &                \cellcolor[rgb]{1.0,0.7468495023281645,0.5} 0.03$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.5837498398052033,0.5} -0.14$\pm$0.15 &                \cellcolor[rgb]{0.8406444171596532,1.0,0.6432265505822823} 0.33$\pm$0.01 &                \cellcolor[rgb]{0.8455556795773338,1.0,0.6383152881646017} 0.26$\pm$0.01 & \cellcolor[rgb]{0.8259106299066116,1.0,0.6579603378353239} 0.65$\pm$0.02 &                \cellcolor[rgb]{0.8283662611154519,1.0,0.6555047066264836} 0.80$\pm$0.03 &                 \cellcolor[rgb]{0.9483201250139524,1.0,0.535550842727983} 0.32$\pm$0.01 &                \cellcolor[rgb]{0.9227220299884659,1.0,0.5611489377534695} 0.39$\pm$0.01 & \cellcolor[rgb]{0.9605982810581537,1.0,0.5232726866837817} 0.25$\pm$0.01 &                \cellcolor[rgb]{0.9276332924061464,1.0,0.5562376753357889} 0.31$\pm$0.01 \\
 Monte Carlo Normalized Sequence Entropy &                 \cellcolor[rgb]{0.990065855564237,0.9743688325003206,0.5} 0.18$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.8157119056773038,0.5} 0.06$\pm$0.10 &                \cellcolor[rgb]{1.0,0.8591994532017602,0.5} 0.06$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.5640138408304499,0.5} -0.15$\pm$0.13 &                               \cellcolor[rgb]{1.0,0.8817548806014783,0.5} 0.09$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.8100730488273743,0.5} -0.10$\pm$0.01 &  \cellcolor[rgb]{0.848011310786174,1.0,0.6358596569557614} 0.62$\pm$0.02 &                \cellcolor[rgb]{0.8736094058116604,1.0,0.6102615619302751} 0.68$\pm$0.03 &                \cellcolor[rgb]{0.8553782044126947,1.0,0.6284927633292406} 0.41$\pm$0.01 &                \cellcolor[rgb]{0.8406444171596532,1.0,0.6432265505822823} 0.47$\pm$0.01 & \cellcolor[rgb]{0.8736094058116604,1.0,0.6102615619302751} 0.31$\pm$0.01 &                \cellcolor[rgb]{0.8858875618558619,1.0,0.5979834058860736} 0.34$\pm$0.01 \\
                        Semantic Entropy &                \cellcolor[rgb]{0.9153551363619451,1.0,0.5685158313799904} 0.22$\pm$0.01 &  \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.16$\pm$0.10 &                \cellcolor[rgb]{1.0,0.7818787645777266,0.5} 0.04$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.635695672604554,0.5} -0.11$\pm$0.14 &                \cellcolor[rgb]{0.8529225732038546,1.0,0.6309483945380809} 0.32$\pm$0.01 &                \cellcolor[rgb]{0.8553782044126947,1.0,0.6284927633292406} 0.25$\pm$0.01 & \cellcolor[rgb]{0.8259106299066116,1.0,0.6579603378353239} 0.65$\pm$0.02 &                 \cellcolor[rgb]{0.8332775235331324,1.0,0.650593444208803} 0.79$\pm$0.03 &                 \cellcolor[rgb]{0.9483201250139524,1.0,0.535550842727983} 0.32$\pm$0.01 &                \cellcolor[rgb]{0.9227220299884659,1.0,0.5611489377534695} 0.39$\pm$0.01 & \cellcolor[rgb]{0.9605982810581537,1.0,0.5232726866837817} 0.25$\pm$0.01 &                \cellcolor[rgb]{0.9276332924061464,1.0,0.5562376753357889} 0.31$\pm$0.01 \\
              Lexical Similarity Rouge-1 &                \cellcolor[rgb]{0.9996874651188749,0.9590755692255117,0.5} 0.17$\pm$0.01 &  \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.15$\pm$0.11 &                \cellcolor[rgb]{1.0,0.9365201418257938,0.5} 0.08$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.8479217395019011,0.5} 0.01$\pm$0.13 &                \cellcolor[rgb]{0.9935632697101611,0.9703532829253707,0.5} 0.17$\pm$0.01 &                 \cellcolor[rgb]{0.9483201250139524,1.0,0.535550842727983} 0.13$\pm$0.02 & \cellcolor[rgb]{0.9655095434758343,1.0,0.5183614242661012} 0.43$\pm$0.03 &                \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.58$\pm$0.04 &                               \cellcolor[rgb]{1.0,0.9477978555256528,0.5} 0.26$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9252424281259346,0.5} 0.28$\pm$0.01 &                \cellcolor[rgb]{1.0,0.8344226579520698,0.5} 0.14$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.7790593361527619,0.5} 0.13$\pm$0.01 \\
              %Lexical Similarity Rouge-2 &                \cellcolor[rgb]{0.9996874651188749,0.9590755692255117,0.5} 0.17$\pm$0.01 &   \cellcolor[rgb]{0.963053912266994,1.0,0.5208170554749414} 0.13$\pm$0.10 &                \cellcolor[rgb]{1.0,0.9365201418257938,0.5} 0.08$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.8157119056773038,0.5} -0.01$\pm$0.15 &                               \cellcolor[rgb]{1.0,0.8157119056773038,0.5} 0.03$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.8100730488273743,0.5} -0.10$\pm$0.01 &                \cellcolor[rgb]{1.0,0.7045580759536932,0.5} 0.02$\pm$0.03 &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.64$\pm$0.07 &                               \cellcolor[rgb]{1.0,0.9477978555256528,0.5} 0.26$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9393395702507584,0.5} 0.29$\pm$0.01 &                \cellcolor[rgb]{1.0,0.8344226579520698,0.5} 0.14$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8128924772523392,0.5} 0.15$\pm$0.01 \\
              Lexical Similarity Rouge-L &                \cellcolor[rgb]{0.9996874651188749,0.9590755692255117,0.5} 0.17$\pm$0.02 &  \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.15$\pm$0.11 &  \cellcolor[rgb]{0.9917773561037317,0.972403776325345,0.5} 0.09$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.8344226579520698,0.5} 0.00$\pm$0.13 &                \cellcolor[rgb]{0.9935632697101611,0.9703532829253707,0.5} 0.17$\pm$0.01 &                 \cellcolor[rgb]{0.9483201250139524,1.0,0.535550842727983} 0.13$\pm$0.01 & \cellcolor[rgb]{0.9655095434758343,1.0,0.5183614242661012} 0.43$\pm$0.03 &                \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.58$\pm$0.04 &                               \cellcolor[rgb]{1.0,0.9337007134008288,0.5} 0.25$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9252424281259346,0.5} 0.28$\pm$0.01 &                \cellcolor[rgb]{1.0,0.8344226579520698,0.5} 0.14$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8128924772523392,0.5} 0.15$\pm$0.01 \\
                 Lexical Similarity BLEU &                               \cellcolor[rgb]{1.0,0.8732965953265841,0.5} 0.13$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.8676577384766544,0.5} 0.08$\pm$0.11 &                \cellcolor[rgb]{1.0,0.9365201418257938,0.5} 0.08$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.7959759067025505,0.5} -0.02$\pm$0.13 &                               \cellcolor[rgb]{1.0,0.9337007134008288,0.5} 0.14$\pm$0.01 & \cellcolor[rgb]{0.9753320683111952,0.9912854030501093,0.5085388994307402} 0.10$\pm$0.02 & \cellcolor[rgb]{0.9655095434758343,1.0,0.5183614242661012} 0.43$\pm$0.03 &                \cellcolor[rgb]{0.9251776611973062,1.0,0.5586933065446292} 0.56$\pm$0.05 &                               \cellcolor[rgb]{1.0,0.9055064291511813,0.5} 0.23$\pm$0.01 &                \cellcolor[rgb]{0.9982140863935707,0.9647144260754412,0.5} 0.31$\pm$0.01 &                \cellcolor[rgb]{1.0,0.8185313341022685,0.5} 0.13$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8298090478021276,0.5} 0.16$\pm$0.01 \\
                              NumSemSets &                               \cellcolor[rgb]{1.0,0.8507411679268658,0.5} 0.12$\pm$0.01 &   \cellcolor[rgb]{0.990065855564237,0.9743688325003206,0.5} 0.12$\pm$0.11 &                \cellcolor[rgb]{1.0,0.7818787645777266,0.5} 0.04$\pm$0.03 &                                \cellcolor[rgb]{1.0,0.956256140800547,0.5} 0.07$\pm$0.15 &                               \cellcolor[rgb]{1.0,0.9111452860011109,0.5} 0.12$\pm$0.01 &                 \cellcolor[rgb]{0.9917773561037317,0.972403776325345,0.5} 0.08$\pm$0.01 & \cellcolor[rgb]{0.9655095434758343,1.0,0.5183614242661012} 0.43$\pm$0.03 &                \cellcolor[rgb]{0.9128995051531048,1.0,0.5709714625888306} 0.59$\pm$0.05 &                               \cellcolor[rgb]{1.0,0.6610705284292367,0.5} 0.03$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.6964415395787946,0.5} 0.08$\pm$0.01 &               \cellcolor[rgb]{1.0,0.5584604212055193,0.5} -0.03$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.5893886966551328,0.5} -0.00$\pm$0.01 \\
       EigValLaplacian NLI Score entail. &                               \cellcolor[rgb]{1.0,0.9365201418257938,0.5} 0.16$\pm$0.01 &   \cellcolor[rgb]{0.990065855564237,0.9743688325003206,0.5} 0.12$\pm$0.11 &                \cellcolor[rgb]{1.0,0.8997821350762528,0.5} 0.07$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.8676577384766544,0.5} 0.02$\pm$0.13 & \cellcolor[rgb]{0.9679651746846745,0.9986330044000171,0.5159057930572609} 0.20$\pm$0.01 &                \cellcolor[rgb]{0.9276332924061464,1.0,0.5562376753357889} 0.16$\pm$0.01 &                \cellcolor[rgb]{1.0,0.9224229997009699,0.5} 0.32$\pm$0.03 &                 \cellcolor[rgb]{0.9311307065520704,1.0,0.552740261189865} 0.53$\pm$0.05 &                               \cellcolor[rgb]{1.0,0.8451023110769363,0.5} 0.18$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8817548806014783,0.5} 0.24$\pm$0.01 &                  \cellcolor[rgb]{1.0,0.80161476355248,0.5} 0.12$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.7959759067025505,0.5} 0.14$\pm$0.01 \\
       EigValLaplacian NLI Score Contra. &                               \cellcolor[rgb]{1.0,0.8732965953265841,0.5} 0.13$\pm$0.01 &   \cellcolor[rgb]{0.963053912266994,1.0,0.5208170554749414} 0.13$\pm$0.11 &                \cellcolor[rgb]{1.0,0.8591994532017602,0.5} 0.06$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.8998675723012518,0.5} 0.04$\pm$0.13 &                \cellcolor[rgb]{0.9876102243553967,0.9771882609252853,0.5} 0.18$\pm$0.01 &                 \cellcolor[rgb]{0.9483201250139524,1.0,0.535550842727983} 0.13$\pm$0.02 &                \cellcolor[rgb]{1.0,0.9449784271006879,0.5} 0.35$\pm$0.03 &                \cellcolor[rgb]{0.9655095434758343,1.0,0.5183614242661012} 0.45$\pm$0.05 &                               \cellcolor[rgb]{1.0,0.8591994532017602,0.5} 0.19$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9393395702507584,0.5} 0.29$\pm$0.01 &                \cellcolor[rgb]{1.0,0.7553077876030589,0.5} 0.09$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.7790593361527619,0.5} 0.13$\pm$0.01 \\
           EigValLaplacian Jaccard Score &                               \cellcolor[rgb]{1.0,0.8732965953265841,0.5} 0.13$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.9506172839506175,0.5} 0.11$\pm$0.11 &  \cellcolor[rgb]{0.9917773561037317,0.972403776325345,0.5} 0.09$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.8344226579520698,0.5} -0.00$\pm$0.13 &                               \cellcolor[rgb]{1.0,0.9337007134008288,0.5} 0.14$\pm$0.01 & \cellcolor[rgb]{0.9851545931465564,0.9800076893502501,0.5002232392008037} 0.09$\pm$0.01 & \cellcolor[rgb]{0.9655095434758343,1.0,0.5183614242661012} 0.43$\pm$0.03 &                \cellcolor[rgb]{0.9128995051531048,1.0,0.5709714625888306} 0.59$\pm$0.04 &                               \cellcolor[rgb]{1.0,0.9196035712760051,0.5} 0.24$\pm$0.01 &                \cellcolor[rgb]{0.9982140863935707,0.9647144260754412,0.5} 0.31$\pm$0.01 &                \cellcolor[rgb]{1.0,0.8344226579520698,0.5} 0.14$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8394634542270069,0.5} 0.17$\pm$0.01 \\
                DegMat NLI Score entail. &                               \cellcolor[rgb]{1.0,0.9365201418257938,0.5} 0.16$\pm$0.02 &  \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.15$\pm$0.11 &                \cellcolor[rgb]{1.0,0.9365201418257938,0.5} 0.08$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.9393395702507584,0.5} 0.06$\pm$0.13 &                               \cellcolor[rgb]{1.0,0.9337007134008288,0.5} 0.14$\pm$0.01 &                \cellcolor[rgb]{0.9996874651188749,0.9590755692255117,0.5} 0.06$\pm$0.01 & \cellcolor[rgb]{0.9384976001785912,1.0,0.5453733675633442} 0.47$\pm$0.03 &                \cellcolor[rgb]{0.9285262492093611,1.0,0.5553447185325744} 0.55$\pm$0.05 &                               \cellcolor[rgb]{1.0,0.8344226579520698,0.5} 0.17$\pm$0.01 &                 \cellcolor[rgb]{0.9917773561037317,0.972403776325345,0.5} 0.32$\pm$0.01 &                \cellcolor[rgb]{1.0,0.8986714511512668,0.5} 0.18$\pm$0.01 & \cellcolor[rgb]{0.9777876995200356,0.9884659746251443,0.5060832682218999} 0.27$\pm$0.01 \\
                DegMat NLI Score Contra. &                               \cellcolor[rgb]{1.0,0.8507411679268658,0.5} 0.12$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.9224229997009699,0.5} 0.10$\pm$0.11 & \cellcolor[rgb]{0.8578338356215351,1.0,0.6260371321204004} 0.13$\pm$0.03 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.19$\pm$0.13 &                               \cellcolor[rgb]{1.0,0.8269896193771629,0.5} 0.04$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.8344226579520698,0.5} -0.07$\pm$0.01 & \cellcolor[rgb]{0.9104438739442646,1.0,0.5734270937976709} 0.52$\pm$0.02 &                 \cellcolor[rgb]{0.936041968969751,1.0,0.5478289987721844} 0.52$\pm$0.04 &                               \cellcolor[rgb]{1.0,0.8451023110769363,0.5} 0.18$\pm$0.01 & \cellcolor[rgb]{0.9826989619377162,0.9828271177752148,0.5020649626074339} 0.33$\pm$0.01 &                \cellcolor[rgb]{1.0,0.8185313341022685,0.5} 0.13$\pm$0.01 &                \cellcolor[rgb]{0.9989507757562228,0.9618949976504765,0.5} 0.25$\pm$0.01 \\
                    DegMat Jaccard Score &                               \cellcolor[rgb]{1.0,0.8732965953265841,0.5} 0.13$\pm$0.02 &                 \cellcolor[rgb]{1.0,0.9506172839506175,0.5} 0.11$\pm$0.11 &                \cellcolor[rgb]{1.0,0.9365201418257938,0.5} 0.08$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.8344226579520698,0.5} -0.00$\pm$0.13 &                               \cellcolor[rgb]{1.0,0.9477978555256528,0.5} 0.15$\pm$0.01 & \cellcolor[rgb]{0.9851545931465564,0.9800076893502501,0.5002232392008037} 0.09$\pm$0.01 & \cellcolor[rgb]{0.9655095434758343,1.0,0.5183614242661012} 0.43$\pm$0.03 &                \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.58$\pm$0.05 &                               \cellcolor[rgb]{1.0,0.8986714511512668,0.5} 0.22$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9506172839506175,0.5} 0.30$\pm$0.01 &                \cellcolor[rgb]{1.0,0.8344226579520698,0.5} 0.14$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8128924772523392,0.5} 0.15$\pm$0.01 \\
          Eccentricity NLI Score entail. &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.27$\pm$0.01 &  \cellcolor[rgb]{0.8455556795773338,1.0,0.6383152881646017} 0.18$\pm$0.11 &                \cellcolor[rgb]{1.0,0.7818787645777266,0.5} 0.04$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.7959759067025505,0.5} -0.02$\pm$0.13 &                 \cellcolor[rgb]{0.820999367488931,1.0,0.6628716002530044} 0.35$\pm$0.01 &                \cellcolor[rgb]{0.8455556795773338,1.0,0.6383152881646017} 0.26$\pm$0.01 & \cellcolor[rgb]{0.9655095434758343,1.0,0.5183614242661012} 0.43$\pm$0.02 &                \cellcolor[rgb]{0.8957100866912229,1.0,0.5881608810507125} 0.63$\pm$0.04 &                \cellcolor[rgb]{0.9996874651188749,0.9590755692255117,0.5} 0.27$\pm$0.01 &                \cellcolor[rgb]{0.9286750753432302,1.0,0.5551958923987053} 0.38$\pm$0.01 &                \cellcolor[rgb]{1.0,0.8986714511512668,0.5} 0.18$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9449784271006879,0.5} 0.24$\pm$0.01 \\
          Eccentricity NLI Score Contra. &                \cellcolor[rgb]{0.9286750753432302,1.0,0.5551958923987053} 0.21$\pm$0.01 &  \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.16$\pm$0.11 &                \cellcolor[rgb]{1.0,0.8997821350762528,0.5} 0.07$\pm$0.03 &                \cellcolor[rgb]{0.8809762994381813,1.0,0.6028946683037542} 0.15$\pm$0.14 & \cellcolor[rgb]{0.9777876995200356,0.9884659746251443,0.5060832682218999} 0.19$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.9477978555256528,0.5} 0.05$\pm$0.01 & \cellcolor[rgb]{0.9458644938051122,1.0,0.5380064739368233} 0.46$\pm$0.03 &                \cellcolor[rgb]{0.9178107675707854,1.0,0.5660602001711501} 0.58$\pm$0.05 &                                \cellcolor[rgb]{1.0,0.884574309026443,0.5} 0.21$\pm$0.01 &  \cellcolor[rgb]{0.9728764371023548,0.994104831475074,0.5109945306395806} 0.34$\pm$0.01 &                \cellcolor[rgb]{1.0,0.8648383100516897,0.5} 0.16$\pm$0.01 &                 \cellcolor[rgb]{0.9917773561037317,0.972403776325345,0.5} 0.26$\pm$0.01 \\
              Eccentricity Jaccard Score &                \cellcolor[rgb]{0.8957100866912229,1.0,0.5881608810507125} 0.23$\pm$0.01 &   \cellcolor[rgb]{0.963053912266994,1.0,0.5208170554749414} 0.13$\pm$0.10 &                \cellcolor[rgb]{1.0,0.8997821350762528,0.5} 0.07$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.7271135033534113,0.5} -0.06$\pm$0.13 &                \cellcolor[rgb]{0.8785206682293409,1.0,0.6053502995125944} 0.29$\pm$0.01 &                \cellcolor[rgb]{0.9030769803177436,1.0,0.5807939874241916} 0.19$\pm$0.01 & \cellcolor[rgb]{0.9655095434758343,1.0,0.5183614242661012} 0.43$\pm$0.03 &                \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.64$\pm$0.05 &                \cellcolor[rgb]{0.9202663987796256,1.0,0.5636045689623098} 0.35$\pm$0.01 &                \cellcolor[rgb]{0.8907988242735423,1.0,0.5930721434683931} 0.42$\pm$0.01 & \cellcolor[rgb]{0.9286750753432302,1.0,0.5551958923987053} 0.27$\pm$0.01 &                \cellcolor[rgb]{0.9128995051531048,1.0,0.5709714625888306} 0.32$\pm$0.01 \\
          Mahalanobis Distance - Decoder &                               \cellcolor[rgb]{1.0,0.6610705284292367,0.5} 0.03$\pm$0.01 &                \cellcolor[rgb]{1.0,0.6238198983297023,0.5} -0.01$\pm$0.11 &                \cellcolor[rgb]{1.0,0.7468495023281645,0.5} 0.03$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.8873937374514077,0.5} 0.03$\pm$0.15 &                               \cellcolor[rgb]{1.0,0.8157119056773038,0.5} 0.03$\pm$0.01 &                 \cellcolor[rgb]{0.9960189009190012,0.967533854500406,0.5} 0.07$\pm$0.01 &                \cellcolor[rgb]{1.0,0.9534367123755823,0.5} 0.36$\pm$0.03 &                \cellcolor[rgb]{0.9202663987796256,1.0,0.5636045689623098} 0.57$\pm$0.05 &                              \cellcolor[rgb]{1.0,0.6006664103549918,0.5} -0.02$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.6063052672049214,0.5} -0.00$\pm$0.01 &                \cellcolor[rgb]{1.0,0.575291554530309,0.5} -0.02$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.5724721261053443,0.5} -0.01$\pm$0.01 \\
 Relative Mahalanobis Distance - Decoder &                               \cellcolor[rgb]{1.0,0.6385151010295187,0.5} 0.02$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.7618010167029778,0.5} 0.04$\pm$0.11 & \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.03$\pm$0.03 &                               \cellcolor[rgb]{1.0,0.707377504378658,0.5} -0.07$\pm$0.12 &                               \cellcolor[rgb]{1.0,0.8157119056773038,0.5} 0.03$\pm$0.01 &                 \cellcolor[rgb]{0.9960189009190012,0.967533854500406,0.5} 0.07$\pm$0.02 & \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.25$\pm$0.04 &                               \cellcolor[rgb]{1.0,0.8213507625272333,0.5} 0.04$\pm$0.08 &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.09$\pm$0.01 &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.08$\pm$0.01 & \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.06$\pm$0.01 &                \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.05$\pm$0.01 \\
                           RDE - Decoder &               \cellcolor[rgb]{0.9996015518506869,0.5374428638557821,0.5} -0.03$\pm$0.01 &  \cellcolor[rgb]{0.9728163992869876,0.514887436456064,0.5} -0.05$\pm$0.11 &                \cellcolor[rgb]{1.0,0.8997821350762528,0.5} 0.07$\pm$0.03 & \cellcolor[rgb]{0.9777876995200356,0.9884659746251443,0.5060832682218999} 0.09$\pm$0.13 &                               \cellcolor[rgb]{1.0,0.8269896193771629,0.5} 0.04$\pm$0.01 & \cellcolor[rgb]{0.9851545931465564,0.9800076893502501,0.5002232392008037} 0.09$\pm$0.02 &                \cellcolor[rgb]{1.0,0.8997821350762528,0.5} 0.29$\pm$0.03 & \cellcolor[rgb]{0.9802433307288758,0.9856465462001796,0.5039066860140641} 0.42$\pm$0.06 &                              \cellcolor[rgb]{1.0,0.6147635524798156,0.5} -0.01$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.5809304113802385,0.5} -0.02$\pm$0.01 &               \cellcolor[rgb]{1.0,0.5950275535050623,0.5} -0.01$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.5584604212055193,0.5} -0.02$\pm$0.01 \\
                        HUQ-MD - Decoder & \cellcolor[rgb]{0.9704208058935146,0.9963774616600456,0.5134501618484207} 0.19$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.8157119056773038,0.5} 0.06$\pm$0.11 &                \cellcolor[rgb]{1.0,0.7468495023281645,0.5} 0.03$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.6554316715793073,0.5} -0.10$\pm$0.14 &                               \cellcolor[rgb]{1.0,0.8817548806014783,0.5} 0.09$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.8732965953265841,0.5} -0.03$\pm$0.02 &  \cellcolor[rgb]{0.848011310786174,1.0,0.6358596569557614} 0.62$\pm$0.02 &                \cellcolor[rgb]{0.8455556795773338,1.0,0.6383152881646017} 0.76$\pm$0.03 & \cellcolor[rgb]{0.9851545931465564,0.9800076893502501,0.5002232392008037} 0.29$\pm$0.01 &                \cellcolor[rgb]{0.9507757562227926,1.0,0.5330952115191427} 0.36$\pm$0.01 & \cellcolor[rgb]{0.9989507757562228,0.9618949976504765,0.5} 0.22$\pm$0.01 &                 \cellcolor[rgb]{0.9917773561037317,0.972403776325345,0.5} 0.26$\pm$0.01 \\
                       HUQ-RMD - Decoder & \cellcolor[rgb]{0.9704208058935146,0.9963774616600456,0.5134501618484207} 0.19$\pm$0.01 &                 \cellcolor[rgb]{1.0,0.8157119056773038,0.5} 0.06$\pm$0.11 &                \cellcolor[rgb]{1.0,0.7045580759536932,0.5} 0.02$\pm$0.03 &                              \cellcolor[rgb]{1.0,0.6034858387799565,0.5} -0.13$\pm$0.14 &                               \cellcolor[rgb]{1.0,0.8817548806014783,0.5} 0.09$\pm$0.01 &                              \cellcolor[rgb]{1.0,0.8732965953265841,0.5} -0.03$\pm$0.01 &                \cellcolor[rgb]{1.0,0.9139647144260756,0.5} 0.31$\pm$0.03 &                \cellcolor[rgb]{0.9079882427354242,1.0,0.5758827250065112} 0.60$\pm$0.05 &                               \cellcolor[rgb]{1.0,0.8986714511512668,0.5} 0.22$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8998675723012518,0.5} 0.26$\pm$0.01 &                \cellcolor[rgb]{1.0,0.9111452860011109,0.5} 0.19$\pm$0.01 &                               \cellcolor[rgb]{1.0,0.8997821350762528,0.5} 0.21$\pm$0.01 \\
\bottomrule
\end{tabular}
}\caption{\label{tab:vicuna_results} PRR$\uparrow$ for the Vicuna model with Rouge-L and BertScore as text quality metrics. Lighter color indicates better results.}\end{table*}

==> tables/dolly_seq.tex <==
\begin{table*}[!ht] \centering\resizebox{0.7\textwidth}{!}{\begin{tabular}{l|c|c|c|c|c|c}
\toprule
\multirow{1}{*}{\textbf{UE Method}} & \textbf{AESLC} & \textbf{XSUM} & \textbf{CoQA} & \textbf{bAbiQA} & \textbf{WMT14 En-De} & \textbf{WMT14 En-Fr}\\ \midrule
\midrule
            Maximum Sequence Probability (baseline) &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.96$\pm$0.01 &       \cellcolor[rgb]{0.5,0.5802475,0.682267} 0.97$\pm$0.01 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.90$\pm$0.00 &  \cellcolor[rgb]{0.8006770000000001,0.7868715,0.732537} 0.73$\pm$0.03 & \cellcolor[rgb]{0.8026055000000001,0.7883884999999999,0.7322204999999999} 0.85$\pm$0.03 &                    \cellcolor[rgb]{0.7443485,0.742659,0.7355039999999999} 0.82$\pm$0.01 \\
                              Perplexity &          \cellcolor[rgb]{0.6548005,0.6701995000000001,0.712395} 0.95$\pm$0.01 &  \cellcolor[rgb]{0.539312,0.606061,0.7190525} 0.95$\pm$0.01 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.90$\pm$0.00 &  \cellcolor[rgb]{0.8006770000000001,0.7868715,0.732537} 0.73$\pm$0.03 &                   \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.86$\pm$0.03 &                    \cellcolor[rgb]{0.6548005,0.6701995000000001,0.712395} 0.84$\pm$0.01 \\
                      Mean Token Entropy &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.96$\pm$0.01 &       \cellcolor[rgb]{0.5,0.5802475,0.682267} 0.97$\pm$0.01 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.90$\pm$0.00 & \cellcolor[rgb]{0.7853034999999999,0.7748475,0.7347965} 0.74$\pm$0.03 &                   \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.86$\pm$0.03 &                    \cellcolor[rgb]{0.6548005,0.6701995000000001,0.712395} 0.84$\pm$0.01 \\
            Pointwise Mutual Information &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.96$\pm$0.01 &   \cellcolor[rgb]{0.574319,0.619862,0.715376} 0.94$\pm$0.02 &                 \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.95$\pm$0.00 &             \cellcolor[rgb]{0.818206,0.800632,0.728909} 0.72$\pm$0.03 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.84$\pm$0.03 &                              \cellcolor[rgb]{0.7910435,0.779335,0.734059} 0.81$\pm$0.02 \\
Conditional Pointwise Mutual Information &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.96$\pm$0.01 &       \cellcolor[rgb]{0.5,0.5802475,0.682267} 0.97$\pm$0.01 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.90$\pm$0.01 &  \cellcolor[rgb]{0.8006770000000001,0.7868715,0.732537} 0.73$\pm$0.03 &                   \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.86$\pm$0.03 &                    \cellcolor[rgb]{0.6548005,0.6701995000000001,0.712395} 0.84$\pm$0.01 \\
                                 P(True) &                   \cellcolor[rgb]{0.516055,0.6005995,0.7203925} 0.97$\pm$0.01 &       \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.98$\pm$0.01 &            \cellcolor[rgb]{0.7910435,0.779335,0.734059} 0.92$\pm$0.00 &            \cellcolor[rgb]{0.8359955,0.814658,0.724009} 0.71$\pm$0.03 & \cellcolor[rgb]{0.8026055000000001,0.7883884999999999,0.7322204999999999} 0.85$\pm$0.04 &                    \cellcolor[rgb]{0.6548005,0.6701995000000001,0.712395} 0.84$\pm$0.01 \\
                        %P(True) Sampling &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.96$\pm$0.01 &       \cellcolor[rgb]{0.5,0.5802475,0.682267} 0.97$\pm$0.01 &            \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.94$\pm$0.00 &            \cellcolor[rgb]{0.8908975,0.858537,0.700983} 0.68$\pm$0.04 &                     \cellcolor[rgb]{0.6886855000000001,0.696202,0.717445} 0.87$\pm$0.03 &                    \cellcolor[rgb]{0.6548005,0.6701995000000001,0.712395} 0.84$\pm$0.01 \\
            Monte Carlo Sequence Entropy &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.98$\pm$0.01 &       \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.98$\pm$0.01 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.90$\pm$0.01 &  \cellcolor[rgb]{0.8006770000000001,0.7868715,0.732537} 0.73$\pm$0.03 & \cellcolor[rgb]{0.8026055000000001,0.7883884999999999,0.7322204999999999} 0.85$\pm$0.04 &                              \cellcolor[rgb]{0.7910435,0.779335,0.734059} 0.81$\pm$0.01 \\
 Monte Carlo Normalized Sequence Entropy &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.98$\pm$0.01 &       \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.98$\pm$0.01 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.90$\pm$0.01 &  \cellcolor[rgb]{0.8006770000000001,0.7868715,0.732537} 0.73$\pm$0.03 & \cellcolor[rgb]{0.8026055000000001,0.7883884999999999,0.7322204999999999} 0.85$\pm$0.04 &                              \cellcolor[rgb]{0.7910435,0.779335,0.734059} 0.81$\pm$0.02 \\
              Lexical Similarity Rouge-1 &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.96$\pm$0.01 &       \cellcolor[rgb]{0.5,0.5934575,0.717766} 0.96$\pm$0.01 & \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.91$\pm$0.00 &            \cellcolor[rgb]{0.8908975,0.858537,0.700983} 0.68$\pm$0.04 &                       \cellcolor[rgb]{0.62987,0.65256,0.7114050000000001} 0.88$\pm$0.03 &                             \cellcolor[rgb]{0.516055,0.6005995,0.7203925} 0.86$\pm$0.01 \\
              Lexical Similarity Rouge-2 & \cellcolor[rgb]{0.700709,0.7058949999999999,0.7203539999999999} 0.94$\pm$0.02 &   \cellcolor[rgb]{0.574319,0.619862,0.715376} 0.94$\pm$0.02 & \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.91$\pm$0.01 &             \cellcolor[rgb]{0.818206,0.800632,0.728909} 0.72$\pm$0.03 &                       \cellcolor[rgb]{0.62987,0.65256,0.7114050000000001} 0.88$\pm$0.03 &                             \cellcolor[rgb]{0.516055,0.6005995,0.7203925} 0.86$\pm$0.01 \\
              Lexical Similarity Rouge-L &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.96$\pm$0.01 &       \cellcolor[rgb]{0.5,0.5934575,0.717766} 0.96$\pm$0.01 & \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.91$\pm$0.01 &            \cellcolor[rgb]{0.8908975,0.858537,0.700983} 0.68$\pm$0.04 &                       \cellcolor[rgb]{0.62987,0.65256,0.7114050000000001} 0.88$\pm$0.03 &                              \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.85$\pm$0.01 \\
                 Lexical Similarity BLEU & \cellcolor[rgb]{0.700709,0.7058949999999999,0.7203539999999999} 0.94$\pm$0.02 &  \cellcolor[rgb]{0.539312,0.606061,0.7190525} 0.95$\pm$0.02 & \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.91$\pm$0.00 &  \cellcolor[rgb]{0.8006770000000001,0.7868715,0.732537} 0.73$\pm$0.03 &                       \cellcolor[rgb]{0.62987,0.65256,0.7114050000000001} 0.88$\pm$0.03 &                             \cellcolor[rgb]{0.516055,0.6005995,0.7203925} 0.86$\pm$0.01 \\
                        Semantic Entropy &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.98$\pm$0.01 &       \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.98$\pm$0.01 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.90$\pm$0.01 &            \cellcolor[rgb]{0.8359955,0.814658,0.724009} 0.71$\pm$0.03 & \cellcolor[rgb]{0.8026055000000001,0.7883884999999999,0.7322204999999999} 0.85$\pm$0.04 &                              \cellcolor[rgb]{0.7910435,0.779335,0.734059} 0.81$\pm$0.02 \\
          Mahalanobis Distance - Decoder &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.96$\pm$0.01 &       \cellcolor[rgb]{0.5,0.5802475,0.682267} 0.97$\pm$0.01 &                 \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.95$\pm$0.00 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.62$\pm$0.04 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.82$\pm$0.04 & \cellcolor[rgb]{0.9484090000000001,0.9055150000000001,0.6604909999999999} 0.78$\pm$0.02 \\
                           RDE - Decoder &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.96$\pm$0.01 &       \cellcolor[rgb]{0.5,0.5802475,0.682267} 0.97$\pm$0.01 &                 \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.95$\pm$0.00 &            \cellcolor[rgb]{0.692134,0.698964,0.7182375} 0.80$\pm$0.03 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.84$\pm$0.04 &          \cellcolor[rgb]{0.8419749999999999,0.8193965000000001,0.7221255} 0.80$\pm$0.01 \\
 Relative Mahalanobis Distance - Decoder &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.96$\pm$0.01 &       \cellcolor[rgb]{0.5,0.5934575,0.717766} 0.96$\pm$0.02 &                 \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.95$\pm$0.00 &          \cellcolor[rgb]{0.6602975,0.6742825,0.7129445} 0.82$\pm$0.03 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.82$\pm$0.04 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.77$\pm$0.02 \\
                        HUQ-MD - Decoder &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.96$\pm$0.01 &       \cellcolor[rgb]{0.5,0.5802475,0.682267} 0.97$\pm$0.03 &            \cellcolor[rgb]{0.7910435,0.779335,0.734059} 0.92$\pm$0.01 &           \cellcolor[rgb]{0.8540335,0.828971,0.7178235} 0.70$\pm$0.03 &                    \cellcolor[rgb]{0.9332104999999999,0.893014,0.6732855} 0.83$\pm$0.04 &                   \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.79$\pm$0.02 \\
                       HUQ-RMD - Decoder &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.96$\pm$0.01 &       \cellcolor[rgb]{0.5,0.5934575,0.717766} 0.96$\pm$0.02 &            \cellcolor[rgb]{0.7910435,0.779335,0.734059} 0.92$\pm$0.00 & \cellcolor[rgb]{0.7058035,0.7100725,0.7217884999999999} 0.79$\pm$0.03 &                    \cellcolor[rgb]{0.9332104999999999,0.893014,0.6732855} 0.83$\pm$0.04 & \cellcolor[rgb]{0.9484090000000001,0.9055150000000001,0.6604909999999999} 0.78$\pm$0.02 \\
           EigValLaplacian Jaccard Score &                    \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.88$\pm$0.01 &  \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.72$\pm$0.03 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.90$\pm$0.03 &                 \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.91$\pm$0.02 & \cellcolor[rgb]{0.8026055000000001,0.7883884999999999,0.7322204999999999} 0.85$\pm$0.04 &          \cellcolor[rgb]{0.8419749999999999,0.8193965000000001,0.7221255} 0.80$\pm$0.03 \\
                    DegMat Jaccard Score &                    \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.88$\pm$0.02 &  \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.72$\pm$0.03 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.90$\pm$0.03 &                 \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.91$\pm$0.01 & \cellcolor[rgb]{0.8026055000000001,0.7883884999999999,0.7322204999999999} 0.85$\pm$0.04 &                              \cellcolor[rgb]{0.7910435,0.779335,0.734059} 0.81$\pm$0.03 \\
              Eccentricity Jaccard Score &         \cellcolor[rgb]{0.8929825,0.8602190000000001,0.6998065} 0.90$\pm$0.01 & \cellcolor[rgb]{0.939689,0.8983435,0.6681205} 0.75$\pm$0.03 &                 \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.95$\pm$0.02 &           \cellcolor[rgb]{0.5231025,0.6019515,0.720098} 0.88$\pm$0.02 &                                   \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.90$\pm$0.03 &                                   \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.87$\pm$0.02 \\
\bottomrule
\end{tabular}
}\caption{\label{tab:dolly_seq_results} RC-AUC$\downarrow$ for the Dolly v2 model with Rouge-L as text quality metrics. Lighter color indicates better results.}\end{table*}

==> tables/dolly_tok.tex <==
\begin{table*}[!ht] \resizebox{\textwidth}{!}{\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{UE Method}} & \multicolumn{2}{c|}{\textbf{AESLC}} & \multicolumn{2}{c|}{\textbf{XSUM}} & \multicolumn{2}{c|}{\textbf{CoQA}} & \multicolumn{2}{c|}{\textbf{bAbiQA}} & \multicolumn{2}{c|}{\textbf{WMT14 En-De}} & \multicolumn{2}{c}{\textbf{WMT14 En-Fr}} \\ %\midrule
\cline{2-13}
    & \textbf{Rouge-L} & \textbf{ModelScore-rh}& \textbf{Rouge-L} & \textbf{ModelScore-rh}& \textbf{Rouge-L} & \textbf{ModelScore-rh}& \textbf{Rouge-L} & \textbf{ModelScore-rh}&  \textbf{Rouge-L} & \textbf{ModelScore-rh}& \textbf{Rouge-L} & \textbf{ModelScore-rh} \\\midrule
\midrule
               Maximum Token Probability & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.62$\pm$0.02 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.98$\pm$0.00 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.52$\pm$0.01 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.94$\pm$0.00 & \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.60$\pm$0.03 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.97$\pm$0.00 & \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.60$\pm$0.01 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.71$\pm$0.03 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.64$\pm$0.02 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.89$\pm$0.00 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.67$\pm$0.02 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.89$\pm$0.00 \\
                                 Entropy & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.62$\pm$0.02 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.98$\pm$0.00 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.52$\pm$0.02 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.93$\pm$0.00 & \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.60$\pm$0.03 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.97$\pm$0.00 & \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.60$\pm$0.01 & \cellcolor[rgb]{0.9484090000000001,0.9055150000000001,0.6604909999999999} 0.72$\pm$0.03 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.64$\pm$0.02 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.89$\pm$0.00 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.67$\pm$0.01 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.89$\pm$0.00 \\
            Pointwise Mutual Information &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.63$\pm$0.02 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.99$\pm$0.00 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.53$\pm$0.01 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.94$\pm$0.00 &                 \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.61$\pm$0.03 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.98$\pm$0.00 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.59$\pm$0.02 &                                   \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.81$\pm$0.02 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.64$\pm$0.02 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.89$\pm$0.00 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.67$\pm$0.02 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.88$\pm$0.00 \\
Conditional Pointwise Mutual Information & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.62$\pm$0.03 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.98$\pm$0.00 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.52$\pm$0.01 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.94$\pm$0.00 & \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.60$\pm$0.03 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.97$\pm$0.00 & \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.60$\pm$0.01 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.71$\pm$0.02 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.64$\pm$0.02 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.89$\pm$0.00 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.67$\pm$0.01 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.89$\pm$0.00 \\
                        Semantic Entropy & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.62$\pm$0.03 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.98$\pm$0.00 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.52$\pm$0.01 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.93$\pm$0.00 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.59$\pm$0.03 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.97$\pm$0.00 &                 \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.61$\pm$0.01 & \cellcolor[rgb]{0.9484090000000001,0.9055150000000001,0.6604909999999999} 0.72$\pm$0.03 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.63$\pm$0.02 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.90$\pm$0.00 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.66$\pm$0.01 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.89$\pm$0.00 \\
\bottomrule
\end{tabular}
}\caption{\label{tab:dolly_tok_results} RC-AUC$\downarrow$ for Dolly v2 model for various tasks for the considered token-level methods. Lighter color indicates better results.}\end{table*}

==> tables/llama_seq.tex <==
\begin{table*}[!ht] \centering\resizebox{0.7\textwidth}{!}{\begin{tabular}{l|c|c|c|c|c|c}
\toprule
\multirow{1}{*}{\textbf{UE Method}} & \textbf{AESLC} & \textbf{XSUM} & \textbf{CoQA} & \textbf{bAbiQA} & \textbf{WMT14 En-De} & \textbf{WMT14 En-Fr}\\ \midrule
\midrule
            Maximum Sequence Probability (baseline) & \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.86$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.74$\pm$0.02 &                   \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.93$\pm$0.00 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.30$\pm$0.03 &                 \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.88$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.86$\pm$0.01 \\
                              Perplexity & \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.86$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.74$\pm$0.02 &                   \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.93$\pm$0.00 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.30$\pm$0.03 &                 \cellcolor[rgb]{0.5,0.595475,0.7205425} 0.87$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.86$\pm$0.01 \\
                      Mean Token Entropy &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.85$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.74$\pm$0.02 &                             \cellcolor[rgb]{0.631869,0.6539155,0.7113945} 0.94$\pm$0.01 &                            \cellcolor[rgb]{0.8826115,0.8518525,0.7052935} 0.37$\pm$0.03 &                 \cellcolor[rgb]{0.5,0.595475,0.7205425} 0.87$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.590805,0.7109295} 0.85$\pm$0.01 \\
            Pointwise Mutual Information & \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.86$\pm$0.01 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.72$\pm$0.03 &                             \cellcolor[rgb]{0.631869,0.6539155,0.7113945} 0.94$\pm$0.00 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.38$\pm$0.03 &  \cellcolor[rgb]{0.671123,0.6824695000000001,0.7142795} 0.84$\pm$0.01 &                  \cellcolor[rgb]{0.6397055,0.6593385,0.7115155} 0.82$\pm$0.01 \\
Conditional Pointwise Mutual Information & \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.86$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.74$\pm$0.02 &                   \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.93$\pm$0.00 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.30$\pm$0.03 &                 \cellcolor[rgb]{0.5,0.595475,0.7205425} 0.87$\pm$0.01 &                         \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.86$\pm$0.01 \\
                                 P(True) & \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.86$\pm$0.01 &                    \cellcolor[rgb]{0.9332104999999999,0.893014,0.6732855} 0.73$\pm$0.02 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.92$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.38$\pm$0.03 &           \cellcolor[rgb]{0.631869,0.6539155,0.7113945} 0.85$\pm$0.01 & \cellcolor[rgb]{0.700709,0.7058949999999999,0.7203539999999999} 0.80$\pm$0.02 \\
                        %P(True) Sampling & \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.88$\pm$0.01 &                    \cellcolor[rgb]{0.9332104999999999,0.893014,0.6732855} 0.73$\pm$0.03 &                   \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.93$\pm$0.00 &            \cellcolor[rgb]{0.96833,0.9219204999999999,0.6404380000000001} 0.32$\pm$0.03 &           \cellcolor[rgb]{0.631869,0.6539155,0.7113945} 0.85$\pm$0.01 &                  \cellcolor[rgb]{0.6397055,0.6593385,0.7115155} 0.82$\pm$0.02 \\
            Monte Carlo Sequence Entropy &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.85$\pm$0.01 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.72$\pm$0.03 &                   \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.93$\pm$0.00 &                    \cellcolor[rgb]{0.820176,0.8021769999999999,0.7283955} 0.41$\pm$0.04 &  \cellcolor[rgb]{0.7443485,0.742659,0.7355039999999999} 0.82$\pm$0.01 &          \cellcolor[rgb]{0.7589600000000001,0.754227,0.7363535} 0.78$\pm$0.02 \\
 Monte Carlo Normalized Sequence Entropy &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.85$\pm$0.01 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.72$\pm$0.03 &                   \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.93$\pm$0.00 &                    \cellcolor[rgb]{0.820176,0.8021769999999999,0.7283955} 0.41$\pm$0.04 &  \cellcolor[rgb]{0.7443485,0.742659,0.7355039999999999} 0.82$\pm$0.01 &          \cellcolor[rgb]{0.7589600000000001,0.754227,0.7363535} 0.78$\pm$0.02 \\
              Lexical Similarity Rouge-1 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.85$\pm$0.01 &                    \cellcolor[rgb]{0.9332104999999999,0.893014,0.6732855} 0.73$\pm$0.03 &                             \cellcolor[rgb]{0.631869,0.6539155,0.7113945} 0.94$\pm$0.00 &                       \cellcolor[rgb]{0.89924,0.86529,0.6962984999999999} 0.36$\pm$0.03 &           \cellcolor[rgb]{0.631869,0.6539155,0.7113945} 0.85$\pm$0.01 & \cellcolor[rgb]{0.700709,0.7058949999999999,0.7203539999999999} 0.80$\pm$0.02 \\
              Lexical Similarity Rouge-2 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.85$\pm$0.01 &                    \cellcolor[rgb]{0.9332104999999999,0.893014,0.6732855} 0.73$\pm$0.03 &                             \cellcolor[rgb]{0.631869,0.6539155,0.7113945} 0.94$\pm$0.00 &                             \cellcolor[rgb]{0.730808,0.7312025,0.7309845} 0.47$\pm$0.03 &  \cellcolor[rgb]{0.671123,0.6824695000000001,0.7142795} 0.84$\pm$0.01 & \cellcolor[rgb]{0.700709,0.7058949999999999,0.7203539999999999} 0.80$\pm$0.02 \\
              Lexical Similarity Rouge-L &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.85$\pm$0.01 &                    \cellcolor[rgb]{0.9332104999999999,0.893014,0.6732855} 0.73$\pm$0.02 &                             \cellcolor[rgb]{0.631869,0.6539155,0.7113945} 0.94$\pm$0.00 &                       \cellcolor[rgb]{0.89924,0.86529,0.6962984999999999} 0.36$\pm$0.04 &  \cellcolor[rgb]{0.671123,0.6824695000000001,0.7142795} 0.84$\pm$0.01 &                    \cellcolor[rgb]{0.729183,0.729776,0.7302285} 0.79$\pm$0.02 \\
                 Lexical Similarity BLEU & \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.86$\pm$0.01 &                    \cellcolor[rgb]{0.9332104999999999,0.893014,0.6732855} 0.73$\pm$0.03 &                             \cellcolor[rgb]{0.631869,0.6539155,0.7113945} 0.94$\pm$0.00 &           \cellcolor[rgb]{0.7159085000000001,0.718475,0.7249909999999999} 0.48$\pm$0.04 &           \cellcolor[rgb]{0.631869,0.6539155,0.7113945} 0.85$\pm$0.01 &          \cellcolor[rgb]{0.671123,0.6824695000000001,0.7142795} 0.81$\pm$0.02 \\
                        Semantic Entropy &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.85$\pm$0.01 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.72$\pm$0.03 &                   \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.93$\pm$0.00 &                              \cellcolor[rgb]{0.850004,0.8257645,0.719312} 0.39$\pm$0.04 &   \cellcolor[rgb]{0.707496,0.7114685000000001,0.722289} 0.83$\pm$0.01 &                    \cellcolor[rgb]{0.729183,0.729776,0.7302285} 0.79$\pm$0.02 \\
          Mahalanobis Distance - Decoder & \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.88$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.74$\pm$0.03 &                                   \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.95$\pm$0.00 &                                   \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.62$\pm$0.03 &   \cellcolor[rgb]{0.707496,0.7114685000000001,0.722289} 0.83$\pm$0.01 &                    \cellcolor[rgb]{0.729183,0.729776,0.7302285} 0.79$\pm$0.02 \\
 Relative Mahalanobis Distance - Decoder & \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.88$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.74$\pm$0.03 &                                   \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.95$\pm$0.00 &                                   \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.62$\pm$0.03 &   \cellcolor[rgb]{0.707496,0.7114685000000001,0.722289} 0.83$\pm$0.01 &          \cellcolor[rgb]{0.7589600000000001,0.754227,0.7363535} 0.78$\pm$0.02 \\
                           RDE - Decoder &           \cellcolor[rgb]{0.824111,0.8052765,0.7274005} 0.87$\pm$0.01 &                    \cellcolor[rgb]{0.9332104999999999,0.893014,0.6732855} 0.73$\pm$0.02 &                                   \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.95$\pm$0.00 &                                   \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.62$\pm$0.03 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.76$\pm$0.02 &                    \cellcolor[rgb]{0.604463,0.636273,0.7124045} 0.83$\pm$0.02 \\
                        HUQ-MD - Decoder & \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.86$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.74$\pm$0.02 &                   \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.93$\pm$0.00 &            \cellcolor[rgb]{0.96833,0.9219204999999999,0.6404380000000001} 0.32$\pm$0.03 &                 \cellcolor[rgb]{0.5,0.595475,0.7205425} 0.87$\pm$0.01 &          \cellcolor[rgb]{0.558806,0.6129675,0.7171540000000001} 0.84$\pm$0.02 \\
                       HUQ-RMD - Decoder & \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.86$\pm$0.01 & \cellcolor[rgb]{0.8662110000000001,0.8386819999999999,0.7128585000000001} 0.74$\pm$0.02 &                   \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.93$\pm$0.00 &            \cellcolor[rgb]{0.96833,0.9219204999999999,0.6404380000000001} 0.32$\pm$0.03 &           \cellcolor[rgb]{0.5825565,0.6239825,0.714454} 0.86$\pm$0.01 &          \cellcolor[rgb]{0.671123,0.6824695000000001,0.7142795} 0.81$\pm$0.02 \\
           EigValLaplacian Jaccard Score &  \cellcolor[rgb]{0.671123,0.6824695000000001,0.7142795} 0.89$\pm$0.01 &                       \cellcolor[rgb]{0.62987,0.65256,0.7114050000000001} 0.78$\pm$0.04 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.91$\pm$0.02 &                              \cellcolor[rgb]{0.834004,0.8130855,0.724635} 0.40$\pm$0.10 & \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.78$\pm$0.05 &  \cellcolor[rgb]{0.96609,0.9200794999999999,0.6429400000000001} 0.72$\pm$0.07 \\
                    DegMat Jaccard Score &  \cellcolor[rgb]{0.671123,0.6824695000000001,0.7142795} 0.89$\pm$0.01 &                       \cellcolor[rgb]{0.62987,0.65256,0.7114050000000001} 0.78$\pm$0.02 &                              \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.91$\pm$0.02 &                              \cellcolor[rgb]{0.834004,0.8130855,0.724635} 0.40$\pm$0.08 & \cellcolor[rgb]{0.9118645000000001,0.8755505,0.6885215} 0.78$\pm$0.06 &                    \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.71$\pm$0.08 \\
              Eccentricity Jaccard Score &                 \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.91$\pm$0.01 &                                   \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.80$\pm$0.02 &                                   \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.95$\pm$0.01 &                              \cellcolor[rgb]{0.834004,0.8130855,0.724635} 0.40$\pm$0.09 &           \cellcolor[rgb]{0.824111,0.8052765,0.7274005} 0.80$\pm$0.07 &                    \cellcolor[rgb]{0.729183,0.729776,0.7302285} 0.79$\pm$0.07 \\
\bottomrule
\end{tabular}
}\caption{\label{tab:llama_seq_results} RC-AUC$\downarrow$ for the Llama v2 model with Rouge-L as text quality metrics. Lighter color indicates better results.}\end{table*}

==> tables/llama_tok.tex <==
\begin{table*}[!ht] \resizebox{\textwidth}{!}{\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{UE Method}} & \multicolumn{2}{c|}{\textbf{AESLC}} & \multicolumn{2}{c|}{\textbf{XSUM}} & \multicolumn{2}{c|}{\textbf{CoQA}} & \multicolumn{2}{c|}{\textbf{bAbiQA}} & \multicolumn{2}{c|}{\textbf{WMT14 En-De}} & \multicolumn{2}{c}{\textbf{WMT14 En-Fr}} \\ %\midrule
\cline{2-13}
    & \textbf{Rouge-L} & \textbf{ModelScore-rh}& \textbf{Rouge-L} & \textbf{ModelScore-rh}& \textbf{Rouge-L} & \textbf{ModelScore-rh}&  \textbf{Rouge-L} & \textbf{ModelScore-rh}& \textbf{Rouge-L} & \textbf{ModelScore-rh}& \textbf{Rouge-L} & \textbf{ModelScore-rh} \\\midrule
\midrule
               Maximum Token Probability & \cellcolor[rgb]{0.7142310000000001,0.71707,0.724432} 0.57$\pm$0.01 & \cellcolor[rgb]{0.516055,0.6005995,0.7203925} 0.90$\pm$0.00 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.50$\pm$0.03 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.94$\pm$0.00 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.65$\pm$0.00 & \cellcolor[rgb]{0.5,0.5776885,0.67525} 0.97$\pm$0.00 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.54$\pm$0.01 & \cellcolor[rgb]{0.501801,0.5979555,0.720782} 0.91$\pm$0.01 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.57$\pm$0.02 & \cellcolor[rgb]{0.516055,0.6005995,0.7203925} 0.90$\pm$0.00 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.52$\pm$0.03 & \cellcolor[rgb]{0.5437325,0.6074395,0.7186710000000001} 0.88$\pm$0.00 \\
                                 Entropy & \cellcolor[rgb]{0.7142310000000001,0.71707,0.724432} 0.57$\pm$0.01 & \cellcolor[rgb]{0.516055,0.6005995,0.7203925} 0.90$\pm$0.00 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.50$\pm$0.03 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.94$\pm$0.00 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.65$\pm$0.00 & \cellcolor[rgb]{0.5,0.5776885,0.67525} 0.97$\pm$0.00 & \cellcolor[rgb]{0.7425705,0.7412255,0.7351920000000001} 0.55$\pm$0.01 & \cellcolor[rgb]{0.501801,0.5979555,0.720782} 0.91$\pm$0.01 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.57$\pm$0.02 & \cellcolor[rgb]{0.516055,0.6005995,0.7203925} 0.90$\pm$0.00 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.52$\pm$0.03 & \cellcolor[rgb]{0.5437325,0.6074395,0.7186710000000001} 0.88$\pm$0.00 \\
            Pointwise Mutual Information & \cellcolor[rgb]{0.7142310000000001,0.71707,0.724432} 0.57$\pm$0.01 & \cellcolor[rgb]{0.516055,0.6005995,0.7203925} 0.90$\pm$0.00 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.49$\pm$0.03 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.93$\pm$0.00 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.66$\pm$0.00 & \cellcolor[rgb]{0.5,0.5776885,0.67525} 0.97$\pm$0.00 &                 \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.56$\pm$0.01 & \cellcolor[rgb]{0.501801,0.5979555,0.720782} 0.91$\pm$0.01 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.56$\pm$0.02 & \cellcolor[rgb]{0.516055,0.6005995,0.7203925} 0.90$\pm$0.00 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.51$\pm$0.03 & \cellcolor[rgb]{0.5437325,0.6074395,0.7186710000000001} 0.88$\pm$0.00 \\
Conditional Pointwise Mutual Information & \cellcolor[rgb]{0.7142310000000001,0.71707,0.724432} 0.57$\pm$0.02 & \cellcolor[rgb]{0.516055,0.6005995,0.7203925} 0.90$\pm$0.00 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.50$\pm$0.03 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.94$\pm$0.00 & \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.65$\pm$0.00 & \cellcolor[rgb]{0.5,0.5776885,0.67525} 0.97$\pm$0.00 &            \cellcolor[rgb]{0.9978685,0.954672,0.608886} 0.54$\pm$0.01 & \cellcolor[rgb]{0.501801,0.5979555,0.720782} 0.91$\pm$0.01 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.57$\pm$0.02 & \cellcolor[rgb]{0.516055,0.6005995,0.7203925} 0.90$\pm$0.00 &      \cellcolor[rgb]{0.5,0.567556,0.6523755} 0.52$\pm$0.03 & \cellcolor[rgb]{0.5437325,0.6074395,0.7186710000000001} 0.88$\pm$0.00 \\
\bottomrule
\end{tabular}
}\caption{\label{tab:llama_tok_results} RC-AUC$\downarrow$ for Llama v2 model for various tasks for the considered sequence-level methods. Lighter color indicates better results.}\end{table*}
